A Total Lagrangian Finite Element Framework for Multibody Dynamics: Part I -- Formulation

We present a Total Lagrangian finite element framework for finite-deformation multibody dynamics. The framework combines a compact kinematic representation, a deformation-gradient-based formulation, an element-agnostic constitutive interface, and a systematic constraint-construction machinery for coupling deformable bodies through engineering joints. Within this setting, we derive the equations of motion for collections of deformable bodies and formulate their response in the presence of external loads, frictional contact forces, and constraint reaction forces. The framework accommodates field forces applied pointwise, over surfaces, or throughout volumes, and supports material models of practical interest, including Mooney-Rivlin, Neo-Hookean, and Kelvin-Voigt. A companion paper discusses the GPU-accelerated implementation of the framework outlined herein and reports on numerical experiments and benchmark results.

==> shape-function-info/beam_22/B_inv_matrix.tex <==
\left[\begin{matrix}\frac{1}{2} & - \frac{3}{2 L} & 0 & \frac{2}{L^{3}}\\\frac{L}{8} & - \frac{1}{4} & - \frac{1}{2 L} & \frac{1}{L^{2}}\\\frac{1}{2} & \frac{3}{2 L} & 0 & - \frac{2}{L^{3}}\\- \frac{L}{8} & - \frac{1}{4} & \frac{1}{2 L} & \frac{1}{L^{2}}\end{matrix}\right]

==> shape-function-info/beam_22/basis_functions.tex <==
\left[\begin{matrix}1\\u\\u^{2}\\u^{3}\end{matrix}\right]

==> shape-function-info/beam_22/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (- \frac{L}{2}, 0, 0) \\
\text{Node 2}: & \quad (\frac{L}{2}, 0, 0) \\
\end{align*}

==> shape-function-info/beam_22/shape_function_derivatives.tex <==
\left[\begin{matrix}- \frac{3}{2 L} + \frac{6 u^{2}}{L^{3}}\\- \frac{1}{4} - \frac{u}{L} + \frac{3 u^{2}}{L^{2}}\\\frac{3}{2 L} - \frac{6 u^{2}}{L^{3}}\\- \frac{1}{4} + \frac{u}{L} + \frac{3 u^{2}}{L^{2}}\end{matrix}\right]

==> shape-function-info/beam_22/shape_functions.tex <==
\left[\begin{matrix}\frac{1}{2} - \frac{3 u}{2 L} + \frac{2 u^{3}}{L^{3}}\\\frac{L}{8} - \frac{u}{4} - \frac{u^{2}}{2 L} + \frac{u^{3}}{L^{2}}\\\frac{1}{2} + \frac{3 u}{2 L} - \frac{2 u^{3}}{L^{3}}\\- \frac{L}{8} - \frac{u}{4} + \frac{u^{2}}{2 L} + \frac{u^{3}}{L^{2}}\end{matrix}\right]

==> shape-function-info/beam_22/verification_matrix.tex <==
\left[\begin{matrix}1 & 0 & 0 & 0\\0 & 1 & 0 & 0\\0 & 0 & 1 & 0\\0 & 0 & 0 & 1\end{matrix}\right]

==> shape-function-info/beam_24/B_inv_matrix.tex <==
\left[\begin{matrix}\frac{1}{2} & - \frac{3}{2 L} & 0 & 0 & 0 & 0 & 0 & \frac{2}{L^{3}}\\\frac{L}{8} & - \frac{1}{4} & 0 & 0 & 0 & 0 & - \frac{1}{2 L} & \frac{1}{L^{2}}\\0 & 0 & \frac{1}{2} & 0 & - \frac{1}{L} & 0 & 0 & 0\\0 & 0 & 0 & \frac{1}{2} & 0 & - \frac{1}{L} & 0 & 0\\\frac{1}{2} & \frac{3}{2 L} & 0 & 0 & 0 & 0 & 0 & - \frac{2}{L^{3}}\\- \frac{L}{8} & - \frac{1}{4} & 0 & 0 & 0 & 0 & \frac{1}{2 L} & \frac{1}{L^{2}}\\0 & 0 & \frac{1}{2} & 0 & \frac{1}{L} & 0 & 0 & 0\\0 & 0 & 0 & \frac{1}{2} & 0 & \frac{1}{L} & 0 & 0\end{matrix}\right]

==> shape-function-info/beam_24/basis_functions.tex <==
\left[\begin{matrix}1\\u\\v\\w\\u v\\u w\\u^{2}\\u^{3}\end{matrix}\right]

==> shape-function-info/beam_24/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (- \frac{L}{2}, 0, 0) \\
\text{Node 2}: & \quad (\frac{L}{2}, 0, 0) \\
\end{align*}

==> shape-function-info/beam_24/shape_function_derivatives.tex <==
\left[\begin{matrix}- \frac{3}{2 L} + \frac{6 u^{2}}{L^{3}} & 0 & 0\\- \frac{1}{4} - \frac{u}{L} + \frac{3 u^{2}}{L^{2}} & 0 & 0\\- \frac{v}{L} & \frac{\frac{L}{2} - u}{L} & 0\\- \frac{w}{L} & 0 & \frac{\frac{L}{2} - u}{L}\\\frac{3}{2 L} - \frac{6 u^{2}}{L^{3}} & 0 & 0\\- \frac{1}{4} + \frac{u}{L} + \frac{3 u^{2}}{L^{2}} & 0 & 0\\\frac{v}{L} & \frac{\frac{L}{2} + u}{L} & 0\\\frac{w}{L} & 0 & \frac{\frac{L}{2} + u}{L}\end{matrix}\right]

==> shape-function-info/beam_24/shape_functions.tex <==
\left[\begin{matrix}\frac{1}{2} - \frac{3 u}{2 L} + \frac{2 u^{3}}{L^{3}}\\\frac{L}{8} - \frac{u}{4} - \frac{u^{2}}{2 L} + \frac{u^{3}}{L^{2}}\\\frac{v}{2} - \frac{u v}{L}\\\frac{w}{2} - \frac{u w}{L}\\\frac{1}{2} + \frac{3 u}{2 L} - \frac{2 u^{3}}{L^{3}}\\- \frac{L}{8} - \frac{u}{4} + \frac{u^{2}}{2 L} + \frac{u^{3}}{L^{2}}\\\frac{v}{2} + \frac{u v}{L}\\\frac{w}{2} + \frac{u w}{L}\end{matrix}\right]

==> shape-function-info/beam_24/verification_matrix.tex <==
\left[\begin{matrix}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{matrix}\right]

==> shape-function-info/beam_34/B_inv_matrix.tex <==
\left[\begin{array}{cccccccccccc}0 & 0 & \frac{4}{L^{2}} & - \frac{10}{L^{3}} & - \frac{8}{L^{4}} & \frac{24}{L^{5}} & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & \frac{1}{2 L} & - \frac{1}{L^{2}} & - \frac{2}{L^{3}} & \frac{4}{L^{4}} & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L} & \frac{2}{L^{2}} & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L} & \frac{2}{L^{2}}\\1 & 0 & - \frac{8}{L^{2}} & 0 & \frac{16}{L^{4}} & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & - \frac{8}{L^{2}} & 0 & \frac{16}{L^{4}} & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & - \frac{4}{L^{2}} & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & - \frac{4}{L^{2}}\\0 & 0 & \frac{4}{L^{2}} & \frac{10}{L^{3}} & - \frac{8}{L^{4}} & - \frac{24}{L^{5}} & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & - \frac{1}{2 L} & - \frac{1}{L^{2}} & \frac{2}{L^{3}} & \frac{4}{L^{4}} & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L} & \frac{2}{L^{2}} & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L} & \frac{2}{L^{2}}\end{array}\right]

==> shape-function-info/beam_34/basis_functions.tex <==
\left[\begin{matrix}1\\u\\u^{2}\\u^{3}\\u^{4}\\u^{5}\\v\\u v\\u^{2} v\\w\\u w\\u^{2} w\end{matrix}\right]

==> shape-function-info/beam_34/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (- \frac{L}{2}, 0, 0) \\
\text{Node 2}: & \quad (0, 0, 0) \\
\text{Node 3}: & \quad (\frac{L}{2}, 0, 0) \\
\end{align*}

==> shape-function-info/beam_34/shape_function_derivatives.tex <==
\left[\begin{matrix}\frac{2 u \left(4 L^{3} - 15 L^{2} u - 16 L u^{2} + 60 u^{3}\right)}{L^{5}} & 0 & 0\\\frac{u \left(L^{3} - 3 L^{2} u - 8 L u^{2} + 20 u^{3}\right)}{L^{4}} & 0 & 0\\\frac{v \left(- L + 4 u\right)}{L^{2}} & \frac{u \left(- L + 2 u\right)}{L^{2}} & 0\\\frac{w \left(- L + 4 u\right)}{L^{2}} & 0 & \frac{u \left(- L + 2 u\right)}{L^{2}}\\\frac{16 u \left(- L^{2} + 4 u^{2}\right)}{L^{4}} & 0 & 0\\1 - \frac{24 u^{2}}{L^{2}} + \frac{80 u^{4}}{L^{4}} & 0 & 0\\- \frac{8 u v}{L^{2}} & 1 - \frac{4 u^{2}}{L^{2}} & 0\\- \frac{8 u w}{L^{2}} & 0 & 1 - \frac{4 u^{2}}{L^{2}}\\\frac{2 u \left(4 L^{3} + 15 L^{2} u - 16 L u^{2} - 60 u^{3}\right)}{L^{5}} & 0 & 0\\\frac{u \left(- L^{3} - 3 L^{2} u + 8 L u^{2} + 20 u^{3}\right)}{L^{4}} & 0 & 0\\\frac{v \left(L + 4 u\right)}{L^{2}} & \frac{u \left(L + 2 u\right)}{L^{2}} & 0\\\frac{w \left(L + 4 u\right)}{L^{2}} & 0 & \frac{u \left(L + 2 u\right)}{L^{2}}\end{matrix}\right]

==> shape-function-info/beam_34/shape_functions.tex <==
\left[\begin{matrix}\frac{4 u^{2}}{L^{2}} - \frac{10 u^{3}}{L^{3}} - \frac{8 u^{4}}{L^{4}} + \frac{24 u^{5}}{L^{5}}\\\frac{u^{2}}{2 L} - \frac{u^{3}}{L^{2}} - \frac{2 u^{4}}{L^{3}} + \frac{4 u^{5}}{L^{4}}\\- \frac{u v}{L} + \frac{2 u^{2} v}{L^{2}}\\- \frac{u w}{L} + \frac{2 u^{2} w}{L^{2}}\\1 - \frac{8 u^{2}}{L^{2}} + \frac{16 u^{4}}{L^{4}}\\u - \frac{8 u^{3}}{L^{2}} + \frac{16 u^{5}}{L^{4}}\\v - \frac{4 u^{2} v}{L^{2}}\\w - \frac{4 u^{2} w}{L^{2}}\\\frac{4 u^{2}}{L^{2}} + \frac{10 u^{3}}{L^{3}} - \frac{8 u^{4}}{L^{4}} - \frac{24 u^{5}}{L^{5}}\\- \frac{u^{2}}{2 L} - \frac{u^{3}}{L^{2}} + \frac{2 u^{4}}{L^{3}} + \frac{4 u^{5}}{L^{4}}\\\frac{u v}{L} + \frac{2 u^{2} v}{L^{2}}\\\frac{u w}{L} + \frac{2 u^{2} w}{L^{2}}\end{matrix}\right]

==> shape-function-info/beam_34/verification_matrix.tex <==
\left[\begin{array}{cccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/hex_27_monomial/B_inv_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & \frac{1}{H W} & - \frac{2}{H^{2} W} & 0 & - \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2} W} & \frac{8}{H^{2} L^{2} W} & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L} & - \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & - \frac{4}{H L W^{2}} & \frac{8}{H^{2} L W^{2}} & 0 & - \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & - \frac{1}{H} & \frac{2}{H^{2}} & 0 & 0 & 0 & 0 & \frac{4}{H W^{2}} & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2}} & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{16}{H L^{2} W^{2}} & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L} & \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & \frac{4}{H L W^{2}} & - \frac{8}{H^{2} L W^{2}} & 0 & - \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{H W} & \frac{2}{H^{2} W} & 0 & - \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2} W} & - \frac{8}{H^{2} L^{2} W} & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & 0 & - \frac{4}{H^{2} L W} & - \frac{2}{L W^{2}} & 0 & \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & - \frac{2}{L^{2} W} & 0 & \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & - \frac{1}{W} & 0 & \frac{4}{H^{2} W} & \frac{2}{W^{2}} & 0 & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{L^{2} W} & 0 & - \frac{16}{H^{2} L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & 0 & \frac{4}{H^{2} L W} & \frac{2}{L W^{2}} & 0 & - \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & - \frac{2}{L^{2} W} & 0 & \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L} & 0 & \frac{4}{H^{2} L} & 0 & 0 & 0 & \frac{4}{L W^{2}} & 0 & - \frac{16}{H^{2} L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\1 & 0 & - \frac{4}{H^{2}} & 0 & 0 & 0 & - \frac{4}{W^{2}} & 0 & \frac{16}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{L^{2}} & 0 & \frac{16}{H^{2} L^{2}} & 0 & 0 & 0 & \frac{16}{L^{2} W^{2}} & 0 & - \frac{64}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L} & 0 & - \frac{4}{H^{2} L} & 0 & 0 & 0 & - \frac{4}{L W^{2}} & 0 & \frac{16}{H^{2} L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & 0 & \frac{4}{H^{2} L W} & - \frac{2}{L W^{2}} & 0 & \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & \frac{2}{L^{2} W} & 0 & - \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & \frac{1}{W} & 0 & - \frac{4}{H^{2} W} & \frac{2}{W^{2}} & 0 & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{L^{2} W} & 0 & \frac{16}{H^{2} L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & 0 & - \frac{4}{H^{2} L W} & \frac{2}{L W^{2}} & 0 & - \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & \frac{2}{L^{2} W} & 0 & - \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{H W} & - \frac{2}{H^{2} W} & 0 & \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2} W} & \frac{8}{H^{2} L^{2} W} & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L} & - \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & \frac{4}{H L W^{2}} & \frac{8}{H^{2} L W^{2}} & 0 & \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & \frac{1}{H} & \frac{2}{H^{2}} & 0 & 0 & 0 & 0 & - \frac{4}{H W^{2}} & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2}} & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{16}{H L^{2} W^{2}} & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L} & \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & - \frac{4}{H L W^{2}} & - \frac{8}{H^{2} L W^{2}} & 0 & \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & \frac{1}{H W} & \frac{2}{H^{2} W} & 0 & \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2} W} & - \frac{8}{H^{2} L^{2} W} & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\end{array}\right]

==> shape-function-info/hex_27_monomial/B_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\- \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2}\\\frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4}\\- \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2}\\\frac{H W}{4} & \frac{H W}{4} & \frac{H W}{4} & 0 & 0 & 0 & - \frac{H W}{4} & - \frac{H W}{4} & - \frac{H W}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H W}{4} & - \frac{H W}{4} & - \frac{H W}{4} & 0 & 0 & 0 & \frac{H W}{4} & \frac{H W}{4} & \frac{H W}{4}\\- \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & 0 & 0 & 0 & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & 0 & 0 & 0 & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & \frac{H^{2} W}{8}\\\frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4}\\- \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & 0 & 0 & 0 & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & 0 & 0 & 0 & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & \frac{H W^{2}}{8}\\\frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16}\\- \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2}\\\frac{H L}{4} & 0 & - \frac{H L}{4} & \frac{H L}{4} & 0 & - \frac{H L}{4} & \frac{H L}{4} & 0 & - \frac{H L}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L}{4} & 0 & \frac{H L}{4} & - \frac{H L}{4} & 0 & \frac{H L}{4} & - \frac{H L}{4} & 0 & \frac{H L}{4}\\- \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8}\\\frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4}\\- \frac{H L W}{8} & 0 & \frac{H L W}{8} & 0 & 0 & 0 & \frac{H L W}{8} & 0 & - \frac{H L W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L W}{8} & 0 & - \frac{H L W}{8} & 0 & 0 & 0 & - \frac{H L W}{8} & 0 & \frac{H L W}{8}\\\frac{H^{2} L W}{16} & 0 & - \frac{H^{2} L W}{16} & 0 & 0 & 0 & - \frac{H^{2} L W}{16} & 0 & \frac{H^{2} L W}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L W}{16} & 0 & - \frac{H^{2} L W}{16} & 0 & 0 & 0 & - \frac{H^{2} L W}{16} & 0 & \frac{H^{2} L W}{16}\\- \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8}\\\frac{H L W^{2}}{16} & 0 & - \frac{H L W^{2}}{16} & 0 & 0 & 0 & \frac{H L W^{2}}{16} & 0 & - \frac{H L W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L W^{2}}{16} & 0 & \frac{H L W^{2}}{16} & 0 & 0 & 0 & - \frac{H L W^{2}}{16} & 0 & \frac{H L W^{2}}{16}\\- \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32}\\\frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4}\\- \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & - \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & - \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8} & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8} & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8}\\\frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16}\\- \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & - \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & - \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8}\\\frac{H L^{2} W}{16} & 0 & \frac{H L^{2} W}{16} & 0 & 0 & 0 & - \frac{H L^{2} W}{16} & 0 & - \frac{H L^{2} W}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L^{2} W}{16} & 0 & - \frac{H L^{2} W}{16} & 0 & 0 & 0 & \frac{H L^{2} W}{16} & 0 & \frac{H L^{2} W}{16}\\- \frac{H^{2} L^{2} W}{32} & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & \frac{H^{2} L^{2} W}{32} & 0 & \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & \frac{H^{2} L^{2} W}{32} & 0 & \frac{H^{2} L^{2} W}{32}\\\frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16}\\- \frac{H L^{2} W^{2}}{32} & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L^{2} W^{2}}{32} & 0 & \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & \frac{H L^{2} W^{2}}{32} & 0 & \frac{H L^{2} W^{2}}{32}\\\frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64}\end{array}\right]

==> shape-function-info/hex_27_monomial/basis_functions.tex <==
\left[\begin{matrix}1\\w\\w^{2}\\v\\v w\\v w^{2}\\v^{2}\\v^{2} w\\v^{2} w^{2}\\u\\u w\\u w^{2}\\u v\\u v w\\u v w^{2}\\u v^{2}\\u v^{2} w\\u v^{2} w^{2}\\u^{2}\\u^{2} w\\u^{2} w^{2}\\u^{2} v\\u^{2} v w\\u^{2} v w^{2}\\u^{2} v^{2}\\u^{2} v^{2} w\\u^{2} v^{2} w^{2}\end{matrix}\right]

==> shape-function-info/hex_27_monomial/node_locations.tex <==
\begin{verbatim}
Node # | (i,j,k) | (u, v, w) coordinates
--------------------------------------------
1      | (0,0,0)     | (-L/2, -W/2, -H/2)
2      | (1,0,0)     | (0, -W/2, -H/2)
3      | (2,0,0)     | (L/2, -W/2, -H/2)
4      | (0,1,0)     | (-L/2, 0, -H/2)
5      | (1,1,0)     | (0, 0, -H/2)
6      | (2,1,0)     | (L/2, 0, -H/2)
7      | (0,2,0)     | (-L/2, W/2, -H/2)
8      | (1,2,0)     | (0, W/2, -H/2)
9      | (2,2,0)     | (L/2, W/2, -H/2)
10     | (0,0,1)     | (-L/2, -W/2, 0)
11     | (1,0,1)     | (0, -W/2, 0)
12     | (2,0,1)     | (L/2, -W/2, 0)
13     | (0,1,1)     | (-L/2, 0, 0)
14     | (1,1,1)     | (0, 0, 0)
15     | (2,1,1)     | (L/2, 0, 0)
16     | (0,2,1)     | (-L/2, W/2, 0)
17     | (1,2,1)     | (0, W/2, 0)
18     | (2,2,1)     | (L/2, W/2, 0)
19     | (0,0,2)     | (-L/2, -W/2, H/2)
20     | (1,0,2)     | (0, -W/2, H/2)
21     | (2,0,2)     | (L/2, -W/2, H/2)
22     | (0,1,2)     | (-L/2, 0, H/2)
23     | (1,1,2)     | (0, 0, H/2)
24     | (2,1,2)     | (L/2, 0, H/2)
25     | (0,2,2)     | (-L/2, W/2, H/2)
26     | (1,2,2)     | (0, W/2, H/2)
27     | (2,2,2)     | (L/2, W/2, H/2)
\end{verbatim}

==> shape-function-info/hex_27_monomial/shape_functions.tex <==
\left[\begin{matrix}- \frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v w}{H W} - \frac{2 v^{2} w}{H W^{2}} - \frac{4 u^{2} v w}{H L^{2} W} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u w}{H L} - \frac{4 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} w}{H L^{2}} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u w^{2}}{H^{2} L} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{w}{H} + \frac{4 v^{2} w}{H W^{2}} + \frac{4 u^{2} w}{H L^{2}} - \frac{16 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 w^{2}}{H^{2}} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u w}{H L} + \frac{4 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} w}{H L^{2}} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u w^{2}}{H^{2} L} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v w}{H W} - \frac{2 v^{2} w}{H W^{2}} + \frac{4 u^{2} v w}{H L^{2} W} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u v w^{2}}{H^{2} L W} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v}{W} + \frac{2 v^{2}}{W^{2}} + \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 v w^{2}}{H^{2} W} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{16 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u v w^{2}}{H^{2} L W} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u}{L} + \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u w^{2}}{H^{2} L} - \frac{16 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\1 - \frac{4 v^{2}}{W^{2}} - \frac{4 u^{2}}{L^{2}} + \frac{16 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 w^{2}}{H^{2}} + \frac{16 v^{2} w^{2}}{H^{2} W^{2}} + \frac{16 u^{2} w^{2}}{H^{2} L^{2}} - \frac{64 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u}{L} - \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u w^{2}}{H^{2} L} + \frac{16 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u v w^{2}}{H^{2} L W} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v}{W} + \frac{2 v^{2}}{W^{2}} - \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 v w^{2}}{H^{2} W} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} + \frac{16 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u v w^{2}}{H^{2} L W} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v w}{H W} + \frac{2 v^{2} w}{H W^{2}} + \frac{4 u^{2} v w}{H L^{2} W} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u w}{H L} + \frac{4 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} w}{H L^{2}} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u w^{2}}{H^{2} L} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{w}{H} - \frac{4 v^{2} w}{H W^{2}} - \frac{4 u^{2} w}{H L^{2}} + \frac{16 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 w^{2}}{H^{2}} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u w}{H L} - \frac{4 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} w}{H L^{2}} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u w^{2}}{H^{2} L} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v w}{H W} + \frac{2 v^{2} w}{H W^{2}} - \frac{4 u^{2} v w}{H L^{2} W} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\end{matrix}\right]

==> shape-function-info/hex_27_monomial/verification_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/hex_q27_lagrange/1D_lagrange_polynomials.tex <==
\left[\begin{matrix}\frac{s \left(s - 1\right)}{2}\\1 - s^{2}\\\frac{s \left(s + 1\right)}{2}\end{matrix}\right]

==> shape-function-info/hex_q27_lagrange/node_locations.tex <==
\begin{verbatim}
Node # | (i,j,k) | (xi, eta, zeta)
----------------------------------
1      | (0,0,0)     | (-1, -1, -1)
2      | (1,0,0)     | ( 0, -1, -1)
3      | (2,0,0)     | ( 1, -1, -1)
4      | (0,1,0)     | (-1,  0, -1)
5      | (1,1,0)     | ( 0,  0, -1)
6      | (2,1,0)     | ( 1,  0, -1)
7      | (0,2,0)     | (-1,  1, -1)
8      | (1,2,0)     | ( 0,  1, -1)
9      | (2,2,0)     | ( 1,  1, -1)
10     | (0,0,1)     | (-1, -1,  0)
11     | (1,0,1)     | ( 0, -1,  0)
12     | (2,0,1)     | ( 1, -1,  0)
13     | (0,1,1)     | (-1,  0,  0)
14     | (1,1,1)     | ( 0,  0,  0)
15     | (2,1,1)     | ( 1,  0,  0)
16     | (0,2,1)     | (-1,  1,  0)
17     | (1,2,1)     | ( 0,  1,  0)
18     | (2,2,1)     | ( 1,  1,  0)
19     | (0,0,2)     | (-1, -1,  1)
20     | (1,0,2)     | ( 0, -1,  1)
21     | (2,0,2)     | ( 1, -1,  1)
22     | (0,1,2)     | (-1,  0,  1)
23     | (1,1,2)     | ( 0,  0,  1)
24     | (2,1,2)     | ( 1,  0,  1)
25     | (0,2,2)     | (-1,  1,  1)
26     | (1,2,2)     | ( 0,  1,  1)
27     | (2,2,2)     | ( 1,  1,  1)
\end{verbatim}

==> shape-function-info/hex_q27_lagrange/shape_functions.tex <==
\left[\begin{matrix}\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} - \frac{\eta^{2} \xi^{2} \zeta}{8} - \frac{\eta^{2} \xi \zeta^{2}}{8} + \frac{\eta^{2} \xi \zeta}{8} - \frac{\eta \xi^{2} \zeta^{2}}{8} + \frac{\eta \xi^{2} \zeta}{8} + \frac{\eta \xi \zeta^{2}}{8} - \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \zeta^{2}}{4} - \frac{\eta^{2} \zeta}{4} + \frac{\eta \xi^{2} \zeta^{2}}{4} - \frac{\eta \xi^{2} \zeta}{4} - \frac{\eta \zeta^{2}}{4} + \frac{\eta \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} - \frac{\eta^{2} \xi^{2} \zeta}{8} + \frac{\eta^{2} \xi \zeta^{2}}{8} - \frac{\eta^{2} \xi \zeta}{8} - \frac{\eta \xi^{2} \zeta^{2}}{8} + \frac{\eta \xi^{2} \zeta}{8} - \frac{\eta \xi \zeta^{2}}{8} + \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \xi \zeta^{2}}{4} - \frac{\eta^{2} \xi \zeta}{4} + \frac{\xi^{2} \zeta^{2}}{4} - \frac{\xi^{2} \zeta}{4} - \frac{\xi \zeta^{2}}{4} + \frac{\xi \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} - \frac{\eta^{2} \xi^{2} \zeta}{2} - \frac{\eta^{2} \zeta^{2}}{2} + \frac{\eta^{2} \zeta}{2} - \frac{\xi^{2} \zeta^{2}}{2} + \frac{\xi^{2} \zeta}{2} + \frac{\zeta^{2}}{2} - \frac{\zeta}{2}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2} \zeta}{4} - \frac{\eta^{2} \xi \zeta^{2}}{4} + \frac{\eta^{2} \xi \zeta}{4} + \frac{\xi^{2} \zeta^{2}}{4} - \frac{\xi^{2} \zeta}{4} + \frac{\xi \zeta^{2}}{4} - \frac{\xi \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} - \frac{\eta^{2} \xi^{2} \zeta}{8} - \frac{\eta^{2} \xi \zeta^{2}}{8} + \frac{\eta^{2} \xi \zeta}{8} + \frac{\eta \xi^{2} \zeta^{2}}{8} - \frac{\eta \xi^{2} \zeta}{8} - \frac{\eta \xi \zeta^{2}}{8} + \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \zeta^{2}}{4} - \frac{\eta^{2} \zeta}{4} - \frac{\eta \xi^{2} \zeta^{2}}{4} + \frac{\eta \xi^{2} \zeta}{4} + \frac{\eta \zeta^{2}}{4} - \frac{\eta \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} - \frac{\eta^{2} \xi^{2} \zeta}{8} + \frac{\eta^{2} \xi \zeta^{2}}{8} - \frac{\eta^{2} \xi \zeta}{8} + \frac{\eta \xi^{2} \zeta^{2}}{8} - \frac{\eta \xi^{2} \zeta}{8} + \frac{\eta \xi \zeta^{2}}{8} - \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2}}{4} + \frac{\eta^{2} \xi \zeta^{2}}{4} - \frac{\eta^{2} \xi}{4} + \frac{\eta \xi^{2} \zeta^{2}}{4} - \frac{\eta \xi^{2}}{4} - \frac{\eta \xi \zeta^{2}}{4} + \frac{\eta \xi}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} - \frac{\eta^{2} \xi^{2}}{2} - \frac{\eta^{2} \zeta^{2}}{2} + \frac{\eta^{2}}{2} - \frac{\eta \xi^{2} \zeta^{2}}{2} + \frac{\eta \xi^{2}}{2} + \frac{\eta \zeta^{2}}{2} - \frac{\eta}{2}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2}}{4} - \frac{\eta^{2} \xi \zeta^{2}}{4} + \frac{\eta^{2} \xi}{4} + \frac{\eta \xi^{2} \zeta^{2}}{4} - \frac{\eta \xi^{2}}{4} + \frac{\eta \xi \zeta^{2}}{4} - \frac{\eta \xi}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} - \frac{\eta^{2} \xi^{2}}{2} - \frac{\eta^{2} \xi \zeta^{2}}{2} + \frac{\eta^{2} \xi}{2} - \frac{\xi^{2} \zeta^{2}}{2} + \frac{\xi^{2}}{2} + \frac{\xi \zeta^{2}}{2} - \frac{\xi}{2}\\- \eta^{2} \xi^{2} \zeta^{2} + \eta^{2} \xi^{2} + \eta^{2} \zeta^{2} - \eta^{2} + \xi^{2} \zeta^{2} - \xi^{2} - \zeta^{2} + 1\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} - \frac{\eta^{2} \xi^{2}}{2} + \frac{\eta^{2} \xi \zeta^{2}}{2} - \frac{\eta^{2} \xi}{2} - \frac{\xi^{2} \zeta^{2}}{2} + \frac{\xi^{2}}{2} - \frac{\xi \zeta^{2}}{2} + \frac{\xi}{2}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2}}{4} + \frac{\eta^{2} \xi \zeta^{2}}{4} - \frac{\eta^{2} \xi}{4} - \frac{\eta \xi^{2} \zeta^{2}}{4} + \frac{\eta \xi^{2}}{4} + \frac{\eta \xi \zeta^{2}}{4} - \frac{\eta \xi}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} - \frac{\eta^{2} \xi^{2}}{2} - \frac{\eta^{2} \zeta^{2}}{2} + \frac{\eta^{2}}{2} + \frac{\eta \xi^{2} \zeta^{2}}{2} - \frac{\eta \xi^{2}}{2} - \frac{\eta \zeta^{2}}{2} + \frac{\eta}{2}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} + \frac{\eta^{2} \xi^{2}}{4} - \frac{\eta^{2} \xi \zeta^{2}}{4} + \frac{\eta^{2} \xi}{4} - \frac{\eta \xi^{2} \zeta^{2}}{4} + \frac{\eta \xi^{2}}{4} - \frac{\eta \xi \zeta^{2}}{4} + \frac{\eta \xi}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} + \frac{\eta^{2} \xi^{2} \zeta}{8} - \frac{\eta^{2} \xi \zeta^{2}}{8} - \frac{\eta^{2} \xi \zeta}{8} - \frac{\eta \xi^{2} \zeta^{2}}{8} - \frac{\eta \xi^{2} \zeta}{8} + \frac{\eta \xi \zeta^{2}}{8} + \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} - \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \zeta^{2}}{4} + \frac{\eta^{2} \zeta}{4} + \frac{\eta \xi^{2} \zeta^{2}}{4} + \frac{\eta \xi^{2} \zeta}{4} - \frac{\eta \zeta^{2}}{4} - \frac{\eta \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} + \frac{\eta^{2} \xi^{2} \zeta}{8} + \frac{\eta^{2} \xi \zeta^{2}}{8} + \frac{\eta^{2} \xi \zeta}{8} - \frac{\eta \xi^{2} \zeta^{2}}{8} - \frac{\eta \xi^{2} \zeta}{8} - \frac{\eta \xi \zeta^{2}}{8} - \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} - \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \xi \zeta^{2}}{4} + \frac{\eta^{2} \xi \zeta}{4} + \frac{\xi^{2} \zeta^{2}}{4} + \frac{\xi^{2} \zeta}{4} - \frac{\xi \zeta^{2}}{4} - \frac{\xi \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{2} + \frac{\eta^{2} \xi^{2} \zeta}{2} - \frac{\eta^{2} \zeta^{2}}{2} - \frac{\eta^{2} \zeta}{2} - \frac{\xi^{2} \zeta^{2}}{2} - \frac{\xi^{2} \zeta}{2} + \frac{\zeta^{2}}{2} + \frac{\zeta}{2}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} - \frac{\eta^{2} \xi^{2} \zeta}{4} - \frac{\eta^{2} \xi \zeta^{2}}{4} - \frac{\eta^{2} \xi \zeta}{4} + \frac{\xi^{2} \zeta^{2}}{4} + \frac{\xi^{2} \zeta}{4} + \frac{\xi \zeta^{2}}{4} + \frac{\xi \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} + \frac{\eta^{2} \xi^{2} \zeta}{8} - \frac{\eta^{2} \xi \zeta^{2}}{8} - \frac{\eta^{2} \xi \zeta}{8} + \frac{\eta \xi^{2} \zeta^{2}}{8} + \frac{\eta \xi^{2} \zeta}{8} - \frac{\eta \xi \zeta^{2}}{8} - \frac{\eta \xi \zeta}{8}\\- \frac{\eta^{2} \xi^{2} \zeta^{2}}{4} - \frac{\eta^{2} \xi^{2} \zeta}{4} + \frac{\eta^{2} \zeta^{2}}{4} + \frac{\eta^{2} \zeta}{4} - \frac{\eta \xi^{2} \zeta^{2}}{4} - \frac{\eta \xi^{2} \zeta}{4} + \frac{\eta \zeta^{2}}{4} + \frac{\eta \zeta}{4}\\\frac{\eta^{2} \xi^{2} \zeta^{2}}{8} + \frac{\eta^{2} \xi^{2} \zeta}{8} + \frac{\eta^{2} \xi \zeta^{2}}{8} + \frac{\eta^{2} \xi \zeta}{8} + \frac{\eta \xi^{2} \zeta^{2}}{8} + \frac{\eta \xi^{2} \zeta}{8} + \frac{\eta \xi \zeta^{2}}{8} + \frac{\eta \xi \zeta}{8}\end{matrix}\right]

==> shape-function-info/hex_q27_lagrange/verification_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/hex_q27_parent/verification_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/hex_q27_reference/B_inv_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & \frac{1}{H W} & - \frac{2}{H^{2} W} & 0 & - \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2} W} & \frac{8}{H^{2} L^{2} W} & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L} & - \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & - \frac{4}{H L W^{2}} & \frac{8}{H^{2} L W^{2}} & 0 & - \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & - \frac{1}{H} & \frac{2}{H^{2}} & 0 & 0 & 0 & 0 & \frac{4}{H W^{2}} & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2}} & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{16}{H L^{2} W^{2}} & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L} & \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & \frac{4}{H L W^{2}} & - \frac{8}{H^{2} L W^{2}} & 0 & - \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{H W} & \frac{2}{H^{2} W} & 0 & - \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2} W} & - \frac{8}{H^{2} L^{2} W} & 0 & \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & - \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & 0 & - \frac{4}{H^{2} L W} & - \frac{2}{L W^{2}} & 0 & \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & - \frac{2}{L^{2} W} & 0 & \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & - \frac{1}{W} & 0 & \frac{4}{H^{2} W} & \frac{2}{W^{2}} & 0 & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{L^{2} W} & 0 & - \frac{16}{H^{2} L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & 0 & \frac{4}{H^{2} L W} & \frac{2}{L W^{2}} & 0 & - \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & - \frac{2}{L^{2} W} & 0 & \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L} & 0 & \frac{4}{H^{2} L} & 0 & 0 & 0 & \frac{4}{L W^{2}} & 0 & - \frac{16}{H^{2} L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\1 & 0 & - \frac{4}{H^{2}} & 0 & 0 & 0 & - \frac{4}{W^{2}} & 0 & \frac{16}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{L^{2}} & 0 & \frac{16}{H^{2} L^{2}} & 0 & 0 & 0 & \frac{16}{L^{2} W^{2}} & 0 & - \frac{64}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L} & 0 & - \frac{4}{H^{2} L} & 0 & 0 & 0 & - \frac{4}{L W^{2}} & 0 & \frac{16}{H^{2} L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & 0 & \frac{4}{H^{2} L W} & - \frac{2}{L W^{2}} & 0 & \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & \frac{2}{L^{2} W} & 0 & - \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & \frac{1}{W} & 0 & - \frac{4}{H^{2} W} & \frac{2}{W^{2}} & 0 & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{L^{2} W} & 0 & \frac{16}{H^{2} L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & 0 & - \frac{4}{H^{2} L W} & \frac{2}{L W^{2}} & 0 & - \frac{8}{H^{2} L W^{2}} & 0 & 0 & 0 & \frac{2}{L^{2} W} & 0 & - \frac{8}{H^{2} L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{H W} & - \frac{2}{H^{2} W} & 0 & \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{H L^{2} W} & \frac{8}{H^{2} L^{2} W} & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & - \frac{2}{H L^{2} W} & - \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L} & - \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & \frac{4}{H L W^{2}} & \frac{8}{H^{2} L W^{2}} & 0 & \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & \frac{1}{H} & \frac{2}{H^{2}} & 0 & 0 & 0 & 0 & - \frac{4}{H W^{2}} & - \frac{8}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2}} & - \frac{8}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & \frac{16}{H L^{2} W^{2}} & \frac{32}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L} & \frac{2}{H^{2} L} & 0 & 0 & 0 & 0 & - \frac{4}{H L W^{2}} & - \frac{8}{H^{2} L W^{2}} & 0 & \frac{2}{H L^{2}} & \frac{4}{H^{2} L^{2}} & 0 & 0 & 0 & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{H L W} & - \frac{2}{H^{2} L W} & 0 & - \frac{2}{H L W^{2}} & - \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & \frac{1}{H W} & \frac{2}{H^{2} W} & 0 & \frac{2}{H W^{2}} & \frac{4}{H^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{4}{H L^{2} W} & - \frac{8}{H^{2} L^{2} W} & 0 & - \frac{8}{H L^{2} W^{2}} & - \frac{16}{H^{2} L^{2} W^{2}}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{H L W} & \frac{2}{H^{2} L W} & 0 & \frac{2}{H L W^{2}} & \frac{4}{H^{2} L W^{2}} & 0 & 0 & 0 & 0 & \frac{2}{H L^{2} W} & \frac{4}{H^{2} L^{2} W} & 0 & \frac{4}{H L^{2} W^{2}} & \frac{8}{H^{2} L^{2} W^{2}}\end{array}\right]

==> shape-function-info/hex_q27_reference/B_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\- \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & - \frac{H}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2} & \frac{H}{2}\\\frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4} & \frac{H^{2}}{4}\\- \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & \frac{W}{2} & \frac{W}{2}\\\frac{H W}{4} & \frac{H W}{4} & \frac{H W}{4} & 0 & 0 & 0 & - \frac{H W}{4} & - \frac{H W}{4} & - \frac{H W}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H W}{4} & - \frac{H W}{4} & - \frac{H W}{4} & 0 & 0 & 0 & \frac{H W}{4} & \frac{H W}{4} & \frac{H W}{4}\\- \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & 0 & 0 & 0 & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & - \frac{H^{2} W}{8} & 0 & 0 & 0 & \frac{H^{2} W}{8} & \frac{H^{2} W}{8} & \frac{H^{2} W}{8}\\\frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & \frac{W^{2}}{4} & \frac{W^{2}}{4}\\- \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & 0 & 0 & 0 & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & - \frac{H W^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & 0 & 0 & 0 & \frac{H W^{2}}{8} & \frac{H W^{2}}{8} & \frac{H W^{2}}{8}\\\frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16} & \frac{H^{2} W^{2}}{16}\\- \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2} & - \frac{L}{2} & 0 & \frac{L}{2}\\\frac{H L}{4} & 0 & - \frac{H L}{4} & \frac{H L}{4} & 0 & - \frac{H L}{4} & \frac{H L}{4} & 0 & - \frac{H L}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L}{4} & 0 & \frac{H L}{4} & - \frac{H L}{4} & 0 & \frac{H L}{4} & - \frac{H L}{4} & 0 & \frac{H L}{4}\\- \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8} & - \frac{H^{2} L}{8} & 0 & \frac{H^{2} L}{8}\\\frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4}\\- \frac{H L W}{8} & 0 & \frac{H L W}{8} & 0 & 0 & 0 & \frac{H L W}{8} & 0 & - \frac{H L W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L W}{8} & 0 & - \frac{H L W}{8} & 0 & 0 & 0 & - \frac{H L W}{8} & 0 & \frac{H L W}{8}\\\frac{H^{2} L W}{16} & 0 & - \frac{H^{2} L W}{16} & 0 & 0 & 0 & - \frac{H^{2} L W}{16} & 0 & \frac{H^{2} L W}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L W}{16} & 0 & - \frac{H^{2} L W}{16} & 0 & 0 & 0 & - \frac{H^{2} L W}{16} & 0 & \frac{H^{2} L W}{16}\\- \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & 0 & 0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8}\\\frac{H L W^{2}}{16} & 0 & - \frac{H L W^{2}}{16} & 0 & 0 & 0 & \frac{H L W^{2}}{16} & 0 & - \frac{H L W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L W^{2}}{16} & 0 & \frac{H L W^{2}}{16} & 0 & 0 & 0 & - \frac{H L W^{2}}{16} & 0 & \frac{H L W^{2}}{16}\\- \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32} & 0 & 0 & 0 & - \frac{H^{2} L W^{2}}{32} & 0 & \frac{H^{2} L W^{2}}{32}\\\frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4}\\- \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & - \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & - \frac{H L^{2}}{8} & 0 & - \frac{H L^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8} & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8} & \frac{H L^{2}}{8} & 0 & \frac{H L^{2}}{8}\\\frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16} & \frac{H^{2} L^{2}}{16} & 0 & \frac{H^{2} L^{2}}{16}\\- \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & - \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & - \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & 0 & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8}\\\frac{H L^{2} W}{16} & 0 & \frac{H L^{2} W}{16} & 0 & 0 & 0 & - \frac{H L^{2} W}{16} & 0 & - \frac{H L^{2} W}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H L^{2} W}{16} & 0 & - \frac{H L^{2} W}{16} & 0 & 0 & 0 & \frac{H L^{2} W}{16} & 0 & \frac{H L^{2} W}{16}\\- \frac{H^{2} L^{2} W}{32} & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & \frac{H^{2} L^{2} W}{32} & 0 & \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & - \frac{H^{2} L^{2} W}{32} & 0 & 0 & 0 & \frac{H^{2} L^{2} W}{32} & 0 & \frac{H^{2} L^{2} W}{32}\\\frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16}\\- \frac{H L^{2} W^{2}}{32} & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & - \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H L^{2} W^{2}}{32} & 0 & \frac{H L^{2} W^{2}}{32} & 0 & 0 & 0 & \frac{H L^{2} W^{2}}{32} & 0 & \frac{H L^{2} W^{2}}{32}\\\frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & 0 & 0 & \frac{H^{2} L^{2} W^{2}}{64} & 0 & \frac{H^{2} L^{2} W^{2}}{64}\end{array}\right]

==> shape-function-info/hex_q27_reference/basis_functions.tex <==
\left[\begin{matrix}1\\w\\w^{2}\\v\\v w\\v w^{2}\\v^{2}\\v^{2} w\\v^{2} w^{2}\\u\\u w\\u w^{2}\\u v\\u v w\\u v w^{2}\\u v^{2}\\u v^{2} w\\u v^{2} w^{2}\\u^{2}\\u^{2} w\\u^{2} w^{2}\\u^{2} v\\u^{2} v w\\u^{2} v w^{2}\\u^{2} v^{2}\\u^{2} v^{2} w\\u^{2} v^{2} w^{2}\end{matrix}\right]

==> shape-function-info/hex_q27_reference/node_locations.tex <==
\begin{verbatim}
Node # | (i,j,k) | (u, v, w) coordinates
--------------------------------------------
1      | (0,0,0)     | (-L/2, -W/2, -H/2)
2      | (1,0,0)     | (0, -W/2, -H/2)
3      | (2,0,0)     | (L/2, -W/2, -H/2)
4      | (0,1,0)     | (-L/2, 0, -H/2)
5      | (1,1,0)     | (0, 0, -H/2)
6      | (2,1,0)     | (L/2, 0, -H/2)
7      | (0,2,0)     | (-L/2, W/2, -H/2)
8      | (1,2,0)     | (0, W/2, -H/2)
9      | (2,2,0)     | (L/2, W/2, -H/2)
10     | (0,0,1)     | (-L/2, -W/2, 0)
11     | (1,0,1)     | (0, -W/2, 0)
12     | (2,0,1)     | (L/2, -W/2, 0)
13     | (0,1,1)     | (-L/2, 0, 0)
14     | (1,1,1)     | (0, 0, 0)
15     | (2,1,1)     | (L/2, 0, 0)
16     | (0,2,1)     | (-L/2, W/2, 0)
17     | (1,2,1)     | (0, W/2, 0)
18     | (2,2,1)     | (L/2, W/2, 0)
19     | (0,0,2)     | (-L/2, -W/2, H/2)
20     | (1,0,2)     | (0, -W/2, H/2)
21     | (2,0,2)     | (L/2, -W/2, H/2)
22     | (0,1,2)     | (-L/2, 0, H/2)
23     | (1,1,2)     | (0, 0, H/2)
24     | (2,1,2)     | (L/2, 0, H/2)
25     | (0,2,2)     | (-L/2, W/2, H/2)
26     | (1,2,2)     | (0, W/2, H/2)
27     | (2,2,2)     | (L/2, W/2, H/2)
\end{verbatim}

==> shape-function-info/hex_q27_reference/shape_function_derivatives.tex <==
\left[\begin{matrix}\frac{v w \left(- H L W + 2 H L v + 4 H W u - 8 H u v + 2 L W w - 4 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(- H L W + 4 H L v + 2 H W u - 8 H u v + 2 L W w - 8 L v w - 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(- H L W + 2 H L v + 2 H W u - 4 H u v + 4 L W w - 8 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v w \left(- H W + 2 H v + 2 W w - 4 v w\right)}{H^{2} L^{2} W^{2}} & \frac{w \left(H L^{2} W - 4 H L^{2} v - 4 H W u^{2} + 16 H u^{2} v - 2 L^{2} W w + 8 L^{2} v w + 8 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}} & \frac{v \left(H L^{2} W - 2 H L^{2} v - 4 H W u^{2} + 8 H u^{2} v - 4 L^{2} W w + 8 L^{2} v w + 16 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(H L W - 2 H L v + 4 H W u - 8 H u v - 2 L W w + 4 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(H L W - 4 H L v + 2 H W u - 8 H u v - 2 L W w + 8 L v w - 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(H L W - 2 H L v + 2 H W u - 4 H u v - 4 L W w + 8 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{w \left(H L W^{2} - 4 H L v^{2} - 4 H W^{2} u + 16 H u v^{2} - 2 L W^{2} w + 8 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(- H L + 2 H u + 2 L w - 4 u w\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(H L W^{2} - 4 H L v^{2} - 2 H W^{2} u + 8 H u v^{2} - 4 L W^{2} w + 16 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u w \left(H W^{2} - 4 H v^{2} - 2 W^{2} w + 8 v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 v w \left(H L^{2} - 4 H u^{2} - 2 L^{2} w + 8 u^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{- H L^{2} W^{2} + 4 H L^{2} v^{2} + 4 H W^{2} u^{2} - 16 H u^{2} v^{2} + 4 L^{2} W^{2} w - 16 L^{2} v^{2} w - 16 W^{2} u^{2} w + 64 u^{2} v^{2} w}{H^{2} L^{2} W^{2}}\\\frac{w \left(- H L W^{2} + 4 H L v^{2} - 4 H W^{2} u + 16 H u v^{2} + 2 L W^{2} w - 8 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(H L + 2 H u - 2 L w - 4 u w\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(- H L W^{2} + 4 H L v^{2} - 2 H W^{2} u + 8 H u v^{2} + 4 L W^{2} w - 16 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(H L W + 2 H L v - 4 H W u - 8 H u v - 2 L W w - 4 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(H L W + 4 H L v - 2 H W u - 8 H u v - 2 L W w - 8 L v w + 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(H L W + 2 H L v - 2 H W u - 4 H u v - 4 L W w - 8 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v w \left(H W + 2 H v - 2 W w - 4 v w\right)}{H^{2} L^{2} W^{2}} & \frac{w \left(- H L^{2} W - 4 H L^{2} v + 4 H W u^{2} + 16 H u^{2} v + 2 L^{2} W w + 8 L^{2} v w - 8 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}} & \frac{v \left(- H L^{2} W - 2 H L^{2} v + 4 H W u^{2} + 8 H u^{2} v + 4 L^{2} W w + 8 L^{2} v w - 16 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(- H L W - 2 H L v - 4 H W u - 8 H u v + 2 L W w + 4 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(- H L W - 4 H L v - 2 H W u - 8 H u v + 2 L W w + 8 L v w + 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(- H L W - 2 H L v - 2 H W u - 4 H u v + 4 L W w + 8 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{v \left(H^{2} L W - 2 H^{2} L v - 4 H^{2} W u + 8 H^{2} u v - 4 L W w^{2} + 8 L v w^{2} + 16 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(H^{2} L W - 4 H^{2} L v - 2 H^{2} W u + 8 H^{2} u v - 4 L W w^{2} + 16 L v w^{2} + 8 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(- L W + 2 L v + 2 W u - 4 u v\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v \left(H^{2} W - 2 H^{2} v - 4 W w^{2} + 8 v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{- H^{2} L^{2} W + 4 H^{2} L^{2} v + 4 H^{2} W u^{2} - 16 H^{2} u^{2} v + 4 L^{2} W w^{2} - 16 L^{2} v w^{2} - 16 W u^{2} w^{2} + 64 u^{2} v w^{2}}{H^{2} L^{2} W^{2}} & \frac{8 v w \left(L^{2} W - 2 L^{2} v - 4 W u^{2} + 8 u^{2} v\right)}{H^{2} L^{2} W^{2}}\\\frac{v \left(- H^{2} L W + 2 H^{2} L v - 4 H^{2} W u + 8 H^{2} u v + 4 L W w^{2} - 8 L v w^{2} + 16 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(- H^{2} L W + 4 H^{2} L v - 2 H^{2} W u + 8 H^{2} u v + 4 L W w^{2} - 16 L v w^{2} + 8 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(L W - 2 L v + 2 W u - 4 u v\right)}{H^{2} L^{2} W^{2}}\\\frac{- H^{2} L W^{2} + 4 H^{2} L v^{2} + 4 H^{2} W^{2} u - 16 H^{2} u v^{2} + 4 L W^{2} w^{2} - 16 L v^{2} w^{2} - 16 W^{2} u w^{2} + 64 u v^{2} w^{2}}{H^{2} L^{2} W^{2}} & \frac{8 u v \left(H^{2} L - 2 H^{2} u - 4 L w^{2} + 8 u w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u w \left(L W^{2} - 4 L v^{2} - 2 W^{2} u + 8 u v^{2}\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u \left(- H^{2} W^{2} + 4 H^{2} v^{2} + 4 W^{2} w^{2} - 16 v^{2} w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 v \left(- H^{2} L^{2} + 4 H^{2} u^{2} + 4 L^{2} w^{2} - 16 u^{2} w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 w \left(- L^{2} W^{2} + 4 L^{2} v^{2} + 4 W^{2} u^{2} - 16 u^{2} v^{2}\right)}{H^{2} L^{2} W^{2}}\\\frac{H^{2} L W^{2} - 4 H^{2} L v^{2} + 4 H^{2} W^{2} u - 16 H^{2} u v^{2} - 4 L W^{2} w^{2} + 16 L v^{2} w^{2} - 16 W^{2} u w^{2} + 64 u v^{2} w^{2}}{H^{2} L^{2} W^{2}} & \frac{8 u v \left(- H^{2} L - 2 H^{2} u + 4 L w^{2} + 8 u w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u w \left(- L W^{2} + 4 L v^{2} - 2 W^{2} u + 8 u v^{2}\right)}{H^{2} L^{2} W^{2}}\\\frac{v \left(- H^{2} L W - 2 H^{2} L v + 4 H^{2} W u + 8 H^{2} u v + 4 L W w^{2} + 8 L v w^{2} - 16 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(- H^{2} L W - 4 H^{2} L v + 2 H^{2} W u + 8 H^{2} u v + 4 L W w^{2} + 16 L v w^{2} - 8 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(L W + 2 L v - 2 W u - 4 u v\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v \left(- H^{2} W - 2 H^{2} v + 4 W w^{2} + 8 v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{H^{2} L^{2} W + 4 H^{2} L^{2} v - 4 H^{2} W u^{2} - 16 H^{2} u^{2} v - 4 L^{2} W w^{2} - 16 L^{2} v w^{2} + 16 W u^{2} w^{2} + 64 u^{2} v w^{2}}{H^{2} L^{2} W^{2}} & \frac{8 v w \left(- L^{2} W - 2 L^{2} v + 4 W u^{2} + 8 u^{2} v\right)}{H^{2} L^{2} W^{2}}\\\frac{v \left(H^{2} L W + 2 H^{2} L v + 4 H^{2} W u + 8 H^{2} u v - 4 L W w^{2} - 8 L v w^{2} - 16 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(H^{2} L W + 4 H^{2} L v + 2 H^{2} W u + 8 H^{2} u v - 4 L W w^{2} - 16 L v w^{2} - 8 W u w^{2} - 32 u v w^{2}\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(- L W - 2 L v - 2 W u - 4 u v\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(H L W - 2 H L v - 4 H W u + 8 H u v + 2 L W w - 4 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(H L W - 4 H L v - 2 H W u + 8 H u v + 2 L W w - 8 L v w - 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(H L W - 2 H L v - 2 H W u + 4 H u v + 4 L W w - 8 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v w \left(H W - 2 H v + 2 W w - 4 v w\right)}{H^{2} L^{2} W^{2}} & \frac{w \left(- H L^{2} W + 4 H L^{2} v + 4 H W u^{2} - 16 H u^{2} v - 2 L^{2} W w + 8 L^{2} v w + 8 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}} & \frac{v \left(- H L^{2} W + 2 H L^{2} v + 4 H W u^{2} - 8 H u^{2} v - 4 L^{2} W w + 8 L^{2} v w + 16 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(- H L W + 2 H L v - 4 H W u + 8 H u v - 2 L W w + 4 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(- H L W + 4 H L v - 2 H W u + 8 H u v - 2 L W w + 8 L v w - 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(- H L W + 2 H L v - 2 H W u + 4 H u v - 4 L W w + 8 L v w - 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{w \left(- H L W^{2} + 4 H L v^{2} + 4 H W^{2} u - 16 H u v^{2} - 2 L W^{2} w + 8 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(H L - 2 H u + 2 L w - 4 u w\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(- H L W^{2} + 4 H L v^{2} + 2 H W^{2} u - 8 H u v^{2} - 4 L W^{2} w + 16 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u w \left(- H W^{2} + 4 H v^{2} - 2 W^{2} w + 8 v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 v w \left(- H L^{2} + 4 H u^{2} - 2 L^{2} w + 8 u^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{H L^{2} W^{2} - 4 H L^{2} v^{2} - 4 H W^{2} u^{2} + 16 H u^{2} v^{2} + 4 L^{2} W^{2} w - 16 L^{2} v^{2} w - 16 W^{2} u^{2} w + 64 u^{2} v^{2} w}{H^{2} L^{2} W^{2}}\\\frac{w \left(H L W^{2} - 4 H L v^{2} + 4 H W^{2} u - 16 H u v^{2} + 2 L W^{2} w - 8 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}} & \frac{8 u v w \left(- H L - 2 H u - 2 L w - 4 u w\right)}{H^{2} L^{2} W^{2}} & \frac{u \left(H L W^{2} - 4 H L v^{2} + 2 H W^{2} u - 8 H u v^{2} + 4 L W^{2} w - 16 L v^{2} w + 8 W^{2} u w - 32 u v^{2} w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(- H L W - 2 H L v + 4 H W u + 8 H u v - 2 L W w - 4 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(- H L W - 4 H L v + 2 H W u + 8 H u v - 2 L W w - 8 L v w + 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(- H L W - 2 H L v + 2 H W u + 4 H u v - 4 L W w - 8 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\\\frac{8 u v w \left(- H W - 2 H v - 2 W w - 4 v w\right)}{H^{2} L^{2} W^{2}} & \frac{w \left(H L^{2} W + 4 H L^{2} v - 4 H W u^{2} - 16 H u^{2} v + 2 L^{2} W w + 8 L^{2} v w - 8 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}} & \frac{v \left(H L^{2} W + 2 H L^{2} v - 4 H W u^{2} - 8 H u^{2} v + 4 L^{2} W w + 8 L^{2} v w - 16 W u^{2} w - 32 u^{2} v w\right)}{H^{2} L^{2} W^{2}}\\\frac{v w \left(H L W + 2 H L v + 4 H W u + 8 H u v + 2 L W w + 4 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u w \left(H L W + 4 H L v + 2 H W u + 8 H u v + 2 L W w + 8 L v w + 4 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}} & \frac{u v \left(H L W + 2 H L v + 2 H W u + 4 H u v + 4 L W w + 8 L v w + 8 W u w + 16 u v w\right)}{H^{2} L^{2} W^{2}}\end{matrix}\right]

==> shape-function-info/hex_q27_reference/shape_functions.tex <==
\left[\begin{matrix}- \frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v w}{H W} - \frac{2 v^{2} w}{H W^{2}} - \frac{4 u^{2} v w}{H L^{2} W} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u w}{H L} - \frac{4 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} w}{H L^{2}} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u w^{2}}{H^{2} L} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{w}{H} + \frac{4 v^{2} w}{H W^{2}} + \frac{4 u^{2} w}{H L^{2}} - \frac{16 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 w^{2}}{H^{2}} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u w}{H L} + \frac{4 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} w}{H L^{2}} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u w^{2}}{H^{2} L} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v w}{H W} - \frac{2 v^{2} w}{H W^{2}} + \frac{4 u^{2} v w}{H L^{2} W} + \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} - \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u v w^{2}}{H^{2} L W} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v}{W} + \frac{2 v^{2}}{W^{2}} + \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 v w^{2}}{H^{2} W} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{16 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u v w^{2}}{H^{2} L W} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u}{L} + \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u w^{2}}{H^{2} L} - \frac{16 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\1 - \frac{4 v^{2}}{W^{2}} - \frac{4 u^{2}}{L^{2}} + \frac{16 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 w^{2}}{H^{2}} + \frac{16 v^{2} w^{2}}{H^{2} W^{2}} + \frac{16 u^{2} w^{2}}{H^{2} L^{2}} - \frac{64 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u}{L} - \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u w^{2}}{H^{2} L} + \frac{16 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} + \frac{4 u v w^{2}}{H^{2} L W} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v}{W} + \frac{2 v^{2}}{W^{2}} - \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 v w^{2}}{H^{2} W} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} + \frac{16 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}} - \frac{4 u v w^{2}}{H^{2} L W} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{v w}{H W} + \frac{2 v^{2} w}{H W^{2}} + \frac{4 u^{2} v w}{H L^{2} W} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} + \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} - \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} - \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u w}{H L} + \frac{4 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} w}{H L^{2}} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u w^{2}}{H^{2} L} + \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{w}{H} - \frac{4 v^{2} w}{H W^{2}} - \frac{4 u^{2} w}{H L^{2}} + \frac{16 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 w^{2}}{H^{2}} - \frac{8 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} w^{2}}{H^{2} L^{2}} + \frac{32 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u w}{H L} - \frac{4 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} w}{H L^{2}} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u w^{2}}{H^{2} L} - \frac{8 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} w^{2}}{H^{2} L^{2}} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\- \frac{u v w}{H L W} - \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} - \frac{2 u v w^{2}}{H^{2} L W} - \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{v w}{H W} + \frac{2 v^{2} w}{H W^{2}} - \frac{4 u^{2} v w}{H L^{2} W} - \frac{8 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 v w^{2}}{H^{2} W} + \frac{4 v^{2} w^{2}}{H^{2} W^{2}} - \frac{8 u^{2} v w^{2}}{H^{2} L^{2} W} - \frac{16 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\\\frac{u v w}{H L W} + \frac{2 u v^{2} w}{H L W^{2}} + \frac{2 u^{2} v w}{H L^{2} W} + \frac{4 u^{2} v^{2} w}{H L^{2} W^{2}} + \frac{2 u v w^{2}}{H^{2} L W} + \frac{4 u v^{2} w^{2}}{H^{2} L W^{2}} + \frac{4 u^{2} v w^{2}}{H^{2} L^{2} W} + \frac{8 u^{2} v^{2} w^{2}}{H^{2} L^{2} W^{2}}\end{matrix}\right]

==> shape-function-info/hex_q27_reference/verification_matrix.tex <==
\left[\begin{array}{ccccccccccccccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/shell_44/B_inv_matrix.tex <==
\left[\begin{array}{cccccccccccccccc}\frac{1}{4} & - \frac{3}{4 L} & - \frac{3}{4 W} & 0 & \frac{2}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L^{3}} & \frac{1}{W^{3}} & - \frac{2}{L^{3} W} & - \frac{2}{L W^{3}}\\\frac{L}{16} & - \frac{1}{8} & - \frac{L}{8 W} & 0 & \frac{1}{4 W} & 0 & 0 & 0 & - \frac{1}{4 L} & 0 & \frac{1}{2 L W} & 0 & \frac{1}{2 L^{2}} & 0 & - \frac{1}{L^{2} W} & 0\\\frac{W}{16} & - \frac{W}{8 L} & - \frac{1}{8} & 0 & \frac{1}{4 L} & 0 & 0 & 0 & 0 & - \frac{1}{4 W} & 0 & \frac{1}{2 L W} & 0 & \frac{1}{2 W^{2}} & 0 & - \frac{1}{L W^{2}}\\0 & 0 & 0 & \frac{1}{4} & 0 & - \frac{1}{2 L} & - \frac{1}{2 W} & \frac{1}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\frac{1}{4} & \frac{3}{4 L} & - \frac{3}{4 W} & 0 & - \frac{2}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L^{3}} & \frac{1}{W^{3}} & \frac{2}{L^{3} W} & \frac{2}{L W^{3}}\\- \frac{L}{16} & - \frac{1}{8} & \frac{L}{8 W} & 0 & \frac{1}{4 W} & 0 & 0 & 0 & \frac{1}{4 L} & 0 & - \frac{1}{2 L W} & 0 & \frac{1}{2 L^{2}} & 0 & - \frac{1}{L^{2} W} & 0\\\frac{W}{16} & \frac{W}{8 L} & - \frac{1}{8} & 0 & - \frac{1}{4 L} & 0 & 0 & 0 & 0 & - \frac{1}{4 W} & 0 & - \frac{1}{2 L W} & 0 & \frac{1}{2 W^{2}} & 0 & \frac{1}{L W^{2}}\\0 & 0 & 0 & \frac{1}{4} & 0 & \frac{1}{2 L} & - \frac{1}{2 W} & - \frac{1}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\frac{1}{4} & \frac{3}{4 L} & \frac{3}{4 W} & 0 & \frac{2}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L^{3}} & - \frac{1}{W^{3}} & - \frac{2}{L^{3} W} & - \frac{2}{L W^{3}}\\- \frac{L}{16} & - \frac{1}{8} & - \frac{L}{8 W} & 0 & - \frac{1}{4 W} & 0 & 0 & 0 & \frac{1}{4 L} & 0 & \frac{1}{2 L W} & 0 & \frac{1}{2 L^{2}} & 0 & \frac{1}{L^{2} W} & 0\\- \frac{W}{16} & - \frac{W}{8 L} & - \frac{1}{8} & 0 & - \frac{1}{4 L} & 0 & 0 & 0 & 0 & \frac{1}{4 W} & 0 & \frac{1}{2 L W} & 0 & \frac{1}{2 W^{2}} & 0 & \frac{1}{L W^{2}}\\0 & 0 & 0 & \frac{1}{4} & 0 & \frac{1}{2 L} & \frac{1}{2 W} & \frac{1}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\frac{1}{4} & - \frac{3}{4 L} & \frac{3}{4 W} & 0 & - \frac{2}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L^{3}} & - \frac{1}{W^{3}} & \frac{2}{L^{3} W} & \frac{2}{L W^{3}}\\\frac{L}{16} & - \frac{1}{8} & \frac{L}{8 W} & 0 & - \frac{1}{4 W} & 0 & 0 & 0 & - \frac{1}{4 L} & 0 & - \frac{1}{2 L W} & 0 & \frac{1}{2 L^{2}} & 0 & \frac{1}{L^{2} W} & 0\\- \frac{W}{16} & \frac{W}{8 L} & - \frac{1}{8} & 0 & \frac{1}{4 L} & 0 & 0 & 0 & 0 & \frac{1}{4 W} & 0 & - \frac{1}{2 L W} & 0 & \frac{1}{2 W^{2}} & 0 & - \frac{1}{L W^{2}}\\0 & 0 & 0 & \frac{1}{4} & 0 & - \frac{1}{2 L} & \frac{1}{2 W} & - \frac{1}{L W} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\end{array}\right]

==> shape-function-info/shell_44/B_matrix.tex <==
\left[\begin{array}{cccccccccccccccc}1 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\- \frac{L}{2} & 1 & 0 & 0 & \frac{L}{2} & 1 & 0 & 0 & \frac{L}{2} & 1 & 0 & 0 & - \frac{L}{2} & 1 & 0 & 0\\- \frac{W}{2} & 0 & 1 & 0 & - \frac{W}{2} & 0 & 1 & 0 & \frac{W}{2} & 0 & 1 & 0 & \frac{W}{2} & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1\\\frac{L W}{4} & - \frac{W}{2} & - \frac{L}{2} & 0 & - \frac{L W}{4} & - \frac{W}{2} & \frac{L}{2} & 0 & \frac{L W}{4} & \frac{W}{2} & \frac{L}{2} & 0 & - \frac{L W}{4} & \frac{W}{2} & - \frac{L}{2} & 0\\0 & 0 & 0 & - \frac{L}{2} & 0 & 0 & 0 & \frac{L}{2} & 0 & 0 & 0 & \frac{L}{2} & 0 & 0 & 0 & - \frac{L}{2}\\0 & 0 & 0 & - \frac{W}{2} & 0 & 0 & 0 & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2}\\0 & 0 & 0 & \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4} & 0 & 0 & 0 & \frac{L W}{4} & 0 & 0 & 0 & - \frac{L W}{4}\\\frac{L^{2}}{4} & - L & 0 & 0 & \frac{L^{2}}{4} & L & 0 & 0 & \frac{L^{2}}{4} & L & 0 & 0 & \frac{L^{2}}{4} & - L & 0 & 0\\\frac{W^{2}}{4} & 0 & - W & 0 & \frac{W^{2}}{4} & 0 & - W & 0 & \frac{W^{2}}{4} & 0 & W & 0 & \frac{W^{2}}{4} & 0 & W & 0\\- \frac{L^{2} W}{8} & \frac{L W}{2} & \frac{L^{2}}{4} & 0 & - \frac{L^{2} W}{8} & - \frac{L W}{2} & \frac{L^{2}}{4} & 0 & \frac{L^{2} W}{8} & \frac{L W}{2} & \frac{L^{2}}{4} & 0 & \frac{L^{2} W}{8} & - \frac{L W}{2} & \frac{L^{2}}{4} & 0\\- \frac{L W^{2}}{8} & \frac{W^{2}}{4} & \frac{L W}{2} & 0 & \frac{L W^{2}}{8} & \frac{W^{2}}{4} & - \frac{L W}{2} & 0 & \frac{L W^{2}}{8} & \frac{W^{2}}{4} & \frac{L W}{2} & 0 & - \frac{L W^{2}}{8} & \frac{W^{2}}{4} & - \frac{L W}{2} & 0\\- \frac{L^{3}}{8} & \frac{3 L^{2}}{4} & 0 & 0 & \frac{L^{3}}{8} & \frac{3 L^{2}}{4} & 0 & 0 & \frac{L^{3}}{8} & \frac{3 L^{2}}{4} & 0 & 0 & - \frac{L^{3}}{8} & \frac{3 L^{2}}{4} & 0 & 0\\- \frac{W^{3}}{8} & 0 & \frac{3 W^{2}}{4} & 0 & - \frac{W^{3}}{8} & 0 & \frac{3 W^{2}}{4} & 0 & \frac{W^{3}}{8} & 0 & \frac{3 W^{2}}{4} & 0 & \frac{W^{3}}{8} & 0 & \frac{3 W^{2}}{4} & 0\\\frac{L^{3} W}{16} & - \frac{3 L^{2} W}{8} & - \frac{L^{3}}{8} & 0 & - \frac{L^{3} W}{16} & - \frac{3 L^{2} W}{8} & \frac{L^{3}}{8} & 0 & \frac{L^{3} W}{16} & \frac{3 L^{2} W}{8} & \frac{L^{3}}{8} & 0 & - \frac{L^{3} W}{16} & \frac{3 L^{2} W}{8} & - \frac{L^{3}}{8} & 0\\\frac{L W^{3}}{16} & - \frac{W^{3}}{8} & - \frac{3 L W^{2}}{8} & 0 & - \frac{L W^{3}}{16} & - \frac{W^{3}}{8} & \frac{3 L W^{2}}{8} & 0 & \frac{L W^{3}}{16} & \frac{W^{3}}{8} & \frac{3 L W^{2}}{8} & 0 & - \frac{L W^{3}}{16} & \frac{W^{3}}{8} & - \frac{3 L W^{2}}{8} & 0\end{array}\right]

==> shape-function-info/shell_44/basis_functions.tex <==
\left[\begin{matrix}1\\u\\v\\w\\u v\\u w\\v w\\u v w\\u^{2}\\v^{2}\\u^{2} v\\u v^{2}\\u^{3}\\v^{3}\\u^{3} v\\u v^{3}\end{matrix}\right]

==> shape-function-info/shell_44/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (- \frac{L}{2}, - \frac{W}{2}, 0) \\
\text{Node 2}: & \quad (\frac{L}{2}, - \frac{W}{2}, 0) \\
\text{Node 3}: & \quad (\frac{L}{2}, \frac{W}{2}, 0) \\
\text{Node 4}: & \quad (- \frac{L}{2}, \frac{W}{2}, 0) \\
\end{align*}

==> shape-function-info/shell_44/shape_function_derivatives.tex <==
\left[\begin{matrix}- \frac{3}{4 L} + \frac{2 v}{L W} - \frac{2 v^{3}}{L W^{3}} + \frac{3 u^{2}}{L^{3}} - \frac{6 u^{2} v}{L^{3} W} & - \frac{3}{4 W} + \frac{3 v^{2}}{W^{3}} + \frac{2 u}{L W} - \frac{6 u v^{2}}{L W^{3}} - \frac{2 u^{3}}{L^{3} W} & 0\\- \frac{1}{8} + \frac{v}{4 W} - \frac{u}{2 L} + \frac{u v}{L W} + \frac{3 u^{2}}{2 L^{2}} - \frac{3 u^{2} v}{L^{2} W} & \frac{\frac{L^{2} \left(- L + 2 u\right)}{8} + \frac{L u^{2}}{2} - u^{3}}{L^{2} W} & 0\\\frac{\frac{W^{2} \left(- W + 2 v\right)}{8} + \frac{W v^{2}}{2} - v^{3}}{L W^{2}} & - \frac{1}{8} - \frac{v}{2 W} + \frac{3 v^{2}}{2 W^{2}} + \frac{u}{4 L} + \frac{u v}{L W} - \frac{3 u v^{2}}{L W^{2}} & 0\\\frac{w \left(- W + 2 v\right)}{2 L W} & \frac{w \left(- L + 2 u\right)}{2 L W} & \frac{1}{4} - \frac{v}{2 W} - \frac{u}{2 L} + \frac{u v}{L W}\\\frac{3}{4 L} - \frac{2 v}{L W} + \frac{2 v^{3}}{L W^{3}} - \frac{3 u^{2}}{L^{3}} + \frac{6 u^{2} v}{L^{3} W} & - \frac{3}{4 W} + \frac{3 v^{2}}{W^{3}} - \frac{2 u}{L W} + \frac{6 u v^{2}}{L W^{3}} + \frac{2 u^{3}}{L^{3} W} & 0\\- \frac{1}{8} + \frac{v}{4 W} + \frac{u}{2 L} - \frac{u v}{L W} + \frac{3 u^{2}}{2 L^{2}} - \frac{3 u^{2} v}{L^{2} W} & \frac{\frac{L^{2} \left(L + 2 u\right)}{8} - \frac{L u^{2}}{2} - u^{3}}{L^{2} W} & 0\\\frac{\frac{W^{2} \left(W - 2 v\right)}{8} - \frac{W v^{2}}{2} + v^{3}}{L W^{2}} & - \frac{1}{8} - \frac{v}{2 W} + \frac{3 v^{2}}{2 W^{2}} - \frac{u}{4 L} - \frac{u v}{L W} + \frac{3 u v^{2}}{L W^{2}} & 0\\\frac{w \left(W - 2 v\right)}{2 L W} & \frac{w \left(- L - 2 u\right)}{2 L W} & \frac{1}{4} - \frac{v}{2 W} + \frac{u}{2 L} - \frac{u v}{L W}\\\frac{3}{4 L} + \frac{2 v}{L W} - \frac{2 v^{3}}{L W^{3}} - \frac{3 u^{2}}{L^{3}} - \frac{6 u^{2} v}{L^{3} W} & \frac{3}{4 W} - \frac{3 v^{2}}{W^{3}} + \frac{2 u}{L W} - \frac{6 u v^{2}}{L W^{3}} - \frac{2 u^{3}}{L^{3} W} & 0\\- \frac{1}{8} - \frac{v}{4 W} + \frac{u}{2 L} + \frac{u v}{L W} + \frac{3 u^{2}}{2 L^{2}} + \frac{3 u^{2} v}{L^{2} W} & \frac{- \frac{L^{2} \left(L + 2 u\right)}{8} + \frac{L u^{2}}{2} + u^{3}}{L^{2} W} & 0\\\frac{- \frac{W^{2} \left(W + 2 v\right)}{8} + \frac{W v^{2}}{2} + v^{3}}{L W^{2}} & - \frac{1}{8} + \frac{v}{2 W} + \frac{3 v^{2}}{2 W^{2}} - \frac{u}{4 L} + \frac{u v}{L W} + \frac{3 u v^{2}}{L W^{2}} & 0\\\frac{w \left(W + 2 v\right)}{2 L W} & \frac{w \left(L + 2 u\right)}{2 L W} & \frac{1}{4} + \frac{v}{2 W} + \frac{u}{2 L} + \frac{u v}{L W}\\- \frac{3}{4 L} - \frac{2 v}{L W} + \frac{2 v^{3}}{L W^{3}} + \frac{3 u^{2}}{L^{3}} + \frac{6 u^{2} v}{L^{3} W} & \frac{3}{4 W} - \frac{3 v^{2}}{W^{3}} - \frac{2 u}{L W} + \frac{6 u v^{2}}{L W^{3}} + \frac{2 u^{3}}{L^{3} W} & 0\\- \frac{1}{8} - \frac{v}{4 W} - \frac{u}{2 L} - \frac{u v}{L W} + \frac{3 u^{2}}{2 L^{2}} + \frac{3 u^{2} v}{L^{2} W} & \frac{\frac{L^{2} \left(L - 2 u\right)}{8} - \frac{L u^{2}}{2} + u^{3}}{L^{2} W} & 0\\\frac{\frac{W^{2} \left(W + 2 v\right)}{8} - \frac{W v^{2}}{2} - v^{3}}{L W^{2}} & - \frac{1}{8} + \frac{v}{2 W} + \frac{3 v^{2}}{2 W^{2}} + \frac{u}{4 L} - \frac{u v}{L W} - \frac{3 u v^{2}}{L W^{2}} & 0\\\frac{w \left(- W - 2 v\right)}{2 L W} & \frac{w \left(L - 2 u\right)}{2 L W} & \frac{1}{4} + \frac{v}{2 W} - \frac{u}{2 L} - \frac{u v}{L W}\end{matrix}\right]

==> shape-function-info/shell_44/shape_functions.tex <==
\left[\begin{matrix}\frac{1}{4} - \frac{3 v}{4 W} + \frac{v^{3}}{W^{3}} - \frac{3 u}{4 L} + \frac{2 u v}{L W} - \frac{2 u v^{3}}{L W^{3}} + \frac{u^{3}}{L^{3}} - \frac{2 u^{3} v}{L^{3} W}\\\frac{L}{16} - \frac{L v}{8 W} - \frac{u}{8} + \frac{u v}{4 W} - \frac{u^{2}}{4 L} + \frac{u^{2} v}{2 L W} + \frac{u^{3}}{2 L^{2}} - \frac{u^{3} v}{L^{2} W}\\\frac{W}{16} - \frac{v}{8} - \frac{v^{2}}{4 W} + \frac{v^{3}}{2 W^{2}} - \frac{W u}{8 L} + \frac{u v}{4 L} + \frac{u v^{2}}{2 L W} - \frac{u v^{3}}{L W^{2}}\\\frac{w}{4} - \frac{v w}{2 W} - \frac{u w}{2 L} + \frac{u v w}{L W}\\\frac{1}{4} - \frac{3 v}{4 W} + \frac{v^{3}}{W^{3}} + \frac{3 u}{4 L} - \frac{2 u v}{L W} + \frac{2 u v^{3}}{L W^{3}} - \frac{u^{3}}{L^{3}} + \frac{2 u^{3} v}{L^{3} W}\\- \frac{L}{16} + \frac{L v}{8 W} - \frac{u}{8} + \frac{u v}{4 W} + \frac{u^{2}}{4 L} - \frac{u^{2} v}{2 L W} + \frac{u^{3}}{2 L^{2}} - \frac{u^{3} v}{L^{2} W}\\\frac{W}{16} - \frac{v}{8} - \frac{v^{2}}{4 W} + \frac{v^{3}}{2 W^{2}} + \frac{W u}{8 L} - \frac{u v}{4 L} - \frac{u v^{2}}{2 L W} + \frac{u v^{3}}{L W^{2}}\\\frac{w}{4} - \frac{v w}{2 W} + \frac{u w}{2 L} - \frac{u v w}{L W}\\\frac{1}{4} + \frac{3 v}{4 W} - \frac{v^{3}}{W^{3}} + \frac{3 u}{4 L} + \frac{2 u v}{L W} - \frac{2 u v^{3}}{L W^{3}} - \frac{u^{3}}{L^{3}} - \frac{2 u^{3} v}{L^{3} W}\\- \frac{L}{16} - \frac{L v}{8 W} - \frac{u}{8} - \frac{u v}{4 W} + \frac{u^{2}}{4 L} + \frac{u^{2} v}{2 L W} + \frac{u^{3}}{2 L^{2}} + \frac{u^{3} v}{L^{2} W}\\- \frac{W}{16} - \frac{v}{8} + \frac{v^{2}}{4 W} + \frac{v^{3}}{2 W^{2}} - \frac{W u}{8 L} - \frac{u v}{4 L} + \frac{u v^{2}}{2 L W} + \frac{u v^{3}}{L W^{2}}\\\frac{w}{4} + \frac{v w}{2 W} + \frac{u w}{2 L} + \frac{u v w}{L W}\\\frac{1}{4} + \frac{3 v}{4 W} - \frac{v^{3}}{W^{3}} - \frac{3 u}{4 L} - \frac{2 u v}{L W} + \frac{2 u v^{3}}{L W^{3}} + \frac{u^{3}}{L^{3}} + \frac{2 u^{3} v}{L^{3} W}\\\frac{L}{16} + \frac{L v}{8 W} - \frac{u}{8} - \frac{u v}{4 W} - \frac{u^{2}}{4 L} - \frac{u^{2} v}{2 L W} + \frac{u^{3}}{2 L^{2}} + \frac{u^{3} v}{L^{2} W}\\- \frac{W}{16} - \frac{v}{8} + \frac{v^{2}}{4 W} + \frac{v^{3}}{2 W^{2}} + \frac{W u}{8 L} + \frac{u v}{4 L} - \frac{u v^{2}}{2 L W} - \frac{u v^{3}}{L W^{2}}\\\frac{w}{4} + \frac{v w}{2 W} - \frac{u w}{2 L} - \frac{u v w}{L W}\end{matrix}\right]

==> shape-function-info/shell_44/verification_matrix.tex <==
\left[\begin{array}{cccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/shell_92/B_inv_matrix.tex <==
\left[\begin{array}{cccccccccccccccccc}0 & 0 & 0 & 0 & \frac{1}{L W} & - \frac{2}{L W^{2}} & 0 & - \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & - \frac{2}{L W^{2}} & 0 & - \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{L W} & \frac{2}{L W^{2}} & 0 & - \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & \frac{2}{L W^{2}} & 0 & - \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}}\\0 & 0 & 0 & 0 & \frac{1}{L W} & \frac{2}{L W^{2}} & 0 & \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L W} & \frac{2}{L W^{2}} & 0 & \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}}\\0 & 0 & 0 & 0 & - \frac{1}{L W} & - \frac{2}{L W^{2}} & 0 & \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L W} & - \frac{2}{L W^{2}} & 0 & \frac{2}{L^{2} W} & \frac{4}{L^{2} W^{2}}\\0 & - \frac{1}{W} & \frac{2}{W^{2}} & 0 & 0 & 0 & 0 & \frac{4}{L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{W} & \frac{2}{W^{2}} & 0 & 0 & 0 & 0 & \frac{4}{L^{2} W} & - \frac{8}{L^{2} W^{2}}\\0 & 0 & 0 & \frac{1}{L} & 0 & - \frac{4}{L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{L} & 0 & - \frac{4}{L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{L^{2} W^{2}}\\0 & \frac{1}{W} & \frac{2}{W^{2}} & 0 & 0 & 0 & 0 & - \frac{4}{L^{2} W} & - \frac{8}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{W} & \frac{2}{W^{2}} & 0 & 0 & 0 & 0 & - \frac{4}{L^{2} W} & - \frac{8}{L^{2} W^{2}}\\0 & 0 & 0 & - \frac{1}{L} & 0 & \frac{4}{L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & - \frac{1}{L} & 0 & \frac{4}{L W^{2}} & \frac{2}{L^{2}} & 0 & - \frac{8}{L^{2} W^{2}}\\1 & 0 & - \frac{4}{W^{2}} & 0 & 0 & 0 & - \frac{4}{L^{2}} & 0 & \frac{16}{L^{2} W^{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & - \frac{4}{W^{2}} & 0 & 0 & 0 & - \frac{4}{L^{2}} & 0 & \frac{16}{L^{2} W^{2}}\end{array}\right]

==> shape-function-info/shell_92/B_matrix.tex <==
\left[\begin{array}{cccccccccccccccccc}1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0\\- \frac{W}{2} & 0 & - \frac{W}{2} & 0 & \frac{W}{2} & 0 & \frac{W}{2} & 0 & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & 0 & 0 & 0 & 0 & 0\\\frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & 0 & 0 & 0 & 0 & 0\\- \frac{L}{2} & 0 & \frac{L}{2} & 0 & \frac{L}{2} & 0 & - \frac{L}{2} & 0 & 0 & 0 & \frac{L}{2} & 0 & 0 & 0 & - \frac{L}{2} & 0 & 0 & 0\\\frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\- \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & - \frac{L W^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & 0 & 0 & \frac{L^{2}}{4} & 0 & 0 & 0 & \frac{L^{2}}{4} & 0 & 0 & 0\\- \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1\\0 & - \frac{W}{2} & 0 & - \frac{W}{2} & 0 & \frac{W}{2} & 0 & \frac{W}{2} & 0 & - \frac{W}{2} & 0 & 0 & 0 & \frac{W}{2} & 0 & 0 & 0 & 0\\0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & \frac{W^{2}}{4} & 0 & 0 & 0 & \frac{W^{2}}{4} & 0 & 0 & 0 & 0\\0 & - \frac{L}{2} & 0 & \frac{L}{2} & 0 & \frac{L}{2} & 0 & - \frac{L}{2} & 0 & 0 & 0 & \frac{L}{2} & 0 & 0 & 0 & - \frac{L}{2} & 0 & 0\\0 & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & \frac{L W}{4} & 0 & - \frac{L W}{4} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & - \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & \frac{L W^{2}}{8} & 0 & - \frac{L W^{2}}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & \frac{L^{2}}{4} & 0 & 0 & 0 & \frac{L^{2}}{4} & 0 & 0 & 0 & \frac{L^{2}}{4} & 0 & 0\\0 & - \frac{L^{2} W}{8} & 0 & - \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & 0 & \frac{L^{2} W}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & \frac{L^{2} W^{2}}{16} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\end{array}\right]

==> shape-function-info/shell_92/basis_functions.tex <==
\left[\begin{matrix}1\\v\\v^{2}\\u\\u v\\u v^{2}\\u^{2}\\u^{2} v\\u^{2} v^{2}\\w\\v w\\v^{2} w\\u w\\u v w\\u v^{2} w\\u^{2} w\\u^{2} v w\\u^{2} v^{2} w\end{matrix}\right]

==> shape-function-info/shell_92/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (- \frac{L}{2}, - \frac{W}{2}, 0) \\
\text{Node 2}: & \quad (\frac{L}{2}, - \frac{W}{2}, 0) \\
\text{Node 3}: & \quad (\frac{L}{2}, \frac{W}{2}, 0) \\
\text{Node 4}: & \quad (- \frac{L}{2}, \frac{W}{2}, 0) \\
\text{Node 5}: & \quad (0, - \frac{W}{2}, 0) \\
\text{Node 6}: & \quad (\frac{L}{2}, 0, 0) \\
\text{Node 7}: & \quad (0, \frac{W}{2}, 0) \\
\text{Node 8}: & \quad (- \frac{L}{2}, 0, 0) \\
\text{Node 9}: & \quad (0, 0, 0) \\
\end{align*}

==> shape-function-info/shell_92/shape_function_derivatives.tex <==
\left[\begin{matrix}\frac{v \left(L W - 2 L v - 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u \left(L W - 4 L v - 2 W u + 8 u v\right)}{L^{2} W^{2}} & 0\\\frac{v w \left(L W - 2 L v - 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u w \left(L W - 4 L v - 2 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u v \left(L W - 2 L v - 2 W u + 4 u v\right)}{L^{2} W^{2}}\\\frac{v \left(- L W + 2 L v - 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u \left(- L W + 4 L v - 2 W u + 8 u v\right)}{L^{2} W^{2}} & 0\\\frac{v w \left(- L W + 2 L v - 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u w \left(- L W + 4 L v - 2 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u v \left(- L W + 2 L v - 2 W u + 4 u v\right)}{L^{2} W^{2}}\\\frac{v \left(L W + 2 L v + 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u \left(L W + 4 L v + 2 W u + 8 u v\right)}{L^{2} W^{2}} & 0\\\frac{v w \left(L W + 2 L v + 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u w \left(L W + 4 L v + 2 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u v \left(L W + 2 L v + 2 W u + 4 u v\right)}{L^{2} W^{2}}\\\frac{v \left(- L W - 2 L v + 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u \left(- L W - 4 L v + 2 W u + 8 u v\right)}{L^{2} W^{2}} & 0\\\frac{v w \left(- L W - 2 L v + 4 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u w \left(- L W - 4 L v + 2 W u + 8 u v\right)}{L^{2} W^{2}} & \frac{u v \left(- L W - 2 L v + 2 W u + 4 u v\right)}{L^{2} W^{2}}\\\frac{8 u v \left(W - 2 v\right)}{L^{2} W^{2}} & \frac{- L^{2} W + 4 L^{2} v + 4 W u^{2} - 16 u^{2} v}{L^{2} W^{2}} & 0\\\frac{8 u v w \left(W - 2 v\right)}{L^{2} W^{2}} & \frac{w \left(- L^{2} W + 4 L^{2} v + 4 W u^{2} - 16 u^{2} v\right)}{L^{2} W^{2}} & \frac{v \left(- L^{2} W + 2 L^{2} v + 4 W u^{2} - 8 u^{2} v\right)}{L^{2} W^{2}}\\\frac{L W^{2} - 4 L v^{2} + 4 W^{2} u - 16 u v^{2}}{L^{2} W^{2}} & \frac{8 u v \left(- L - 2 u\right)}{L^{2} W^{2}} & 0\\\frac{w \left(L W^{2} - 4 L v^{2} + 4 W^{2} u - 16 u v^{2}\right)}{L^{2} W^{2}} & \frac{8 u v w \left(- L - 2 u\right)}{L^{2} W^{2}} & \frac{u \left(L W^{2} - 4 L v^{2} + 2 W^{2} u - 8 u v^{2}\right)}{L^{2} W^{2}}\\\frac{8 u v \left(- W - 2 v\right)}{L^{2} W^{2}} & \frac{L^{2} W + 4 L^{2} v - 4 W u^{2} - 16 u^{2} v}{L^{2} W^{2}} & 0\\\frac{8 u v w \left(- W - 2 v\right)}{L^{2} W^{2}} & \frac{w \left(L^{2} W + 4 L^{2} v - 4 W u^{2} - 16 u^{2} v\right)}{L^{2} W^{2}} & \frac{v \left(L^{2} W + 2 L^{2} v - 4 W u^{2} - 8 u^{2} v\right)}{L^{2} W^{2}}\\\frac{- L W^{2} + 4 L v^{2} + 4 W^{2} u - 16 u v^{2}}{L^{2} W^{2}} & \frac{8 u v \left(L - 2 u\right)}{L^{2} W^{2}} & 0\\\frac{w \left(- L W^{2} + 4 L v^{2} + 4 W^{2} u - 16 u v^{2}\right)}{L^{2} W^{2}} & \frac{8 u v w \left(L - 2 u\right)}{L^{2} W^{2}} & \frac{u \left(- L W^{2} + 4 L v^{2} + 2 W^{2} u - 8 u v^{2}\right)}{L^{2} W^{2}}\\\frac{8 u \left(- W^{2} + 4 v^{2}\right)}{L^{2} W^{2}} & \frac{8 v \left(- L^{2} + 4 u^{2}\right)}{L^{2} W^{2}} & 0\\\frac{8 u w \left(- W^{2} + 4 v^{2}\right)}{L^{2} W^{2}} & \frac{8 v w \left(- L^{2} + 4 u^{2}\right)}{L^{2} W^{2}} & 1 - \frac{4 v^{2}}{W^{2}} - \frac{4 u^{2}}{L^{2}} + \frac{16 u^{2} v^{2}}{L^{2} W^{2}}\end{matrix}\right]

==> shape-function-info/shell_92/shape_functions.tex <==
\left[\begin{matrix}\frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}}\\\frac{u v w}{L W} - \frac{2 u v^{2} w}{L W^{2}} - \frac{2 u^{2} v w}{L^{2} W} + \frac{4 u^{2} v^{2} w}{L^{2} W^{2}}\\- \frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} - \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}}\\- \frac{u v w}{L W} + \frac{2 u v^{2} w}{L W^{2}} - \frac{2 u^{2} v w}{L^{2} W} + \frac{4 u^{2} v^{2} w}{L^{2} W^{2}}\\\frac{u v}{L W} + \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}}\\\frac{u v w}{L W} + \frac{2 u v^{2} w}{L W^{2}} + \frac{2 u^{2} v w}{L^{2} W} + \frac{4 u^{2} v^{2} w}{L^{2} W^{2}}\\- \frac{u v}{L W} - \frac{2 u v^{2}}{L W^{2}} + \frac{2 u^{2} v}{L^{2} W} + \frac{4 u^{2} v^{2}}{L^{2} W^{2}}\\- \frac{u v w}{L W} - \frac{2 u v^{2} w}{L W^{2}} + \frac{2 u^{2} v w}{L^{2} W} + \frac{4 u^{2} v^{2} w}{L^{2} W^{2}}\\- \frac{v}{W} + \frac{2 v^{2}}{W^{2}} + \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}}\\- \frac{v w}{W} + \frac{2 v^{2} w}{W^{2}} + \frac{4 u^{2} v w}{L^{2} W} - \frac{8 u^{2} v^{2} w}{L^{2} W^{2}}\\\frac{u}{L} - \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}}\\\frac{u w}{L} - \frac{4 u v^{2} w}{L W^{2}} + \frac{2 u^{2} w}{L^{2}} - \frac{8 u^{2} v^{2} w}{L^{2} W^{2}}\\\frac{v}{W} + \frac{2 v^{2}}{W^{2}} - \frac{4 u^{2} v}{L^{2} W} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}}\\\frac{v w}{W} + \frac{2 v^{2} w}{W^{2}} - \frac{4 u^{2} v w}{L^{2} W} - \frac{8 u^{2} v^{2} w}{L^{2} W^{2}}\\- \frac{u}{L} + \frac{4 u v^{2}}{L W^{2}} + \frac{2 u^{2}}{L^{2}} - \frac{8 u^{2} v^{2}}{L^{2} W^{2}}\\- \frac{u w}{L} + \frac{4 u v^{2} w}{L W^{2}} + \frac{2 u^{2} w}{L^{2}} - \frac{8 u^{2} v^{2} w}{L^{2} W^{2}}\\1 - \frac{4 v^{2}}{W^{2}} - \frac{4 u^{2}}{L^{2}} + \frac{16 u^{2} v^{2}}{L^{2} W^{2}}\\w - \frac{4 v^{2} w}{W^{2}} - \frac{4 u^{2} w}{L^{2}} + \frac{16 u^{2} v^{2} w}{L^{2} W^{2}}\end{matrix}\right]

==> shape-function-info/shell_92/verification_matrix.tex <==
\left[\begin{array}{cccccccccccccccccc}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{array}\right]

==> shape-function-info/tet10_parent/verification_matrix.tex <==
\left[\begin{matrix}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{matrix}\right]

==> shape-function-info/tet10_reference/B_inv_matrix.tex <==
\left[\begin{matrix}1 & - \frac{3}{a} & - \frac{3}{b} & - \frac{3}{c} & \frac{4}{a b} & \frac{4}{a c} & \frac{4}{b c} & \frac{2}{a^{2}} & \frac{2}{b^{2}} & \frac{2}{c^{2}}\\0 & - \frac{1}{a} & 0 & 0 & 0 & 0 & 0 & \frac{2}{a^{2}} & 0 & 0\\0 & 0 & - \frac{1}{b} & 0 & 0 & 0 & 0 & 0 & \frac{2}{b^{2}} & 0\\0 & 0 & 0 & - \frac{1}{c} & 0 & 0 & 0 & 0 & 0 & \frac{2}{c^{2}}\\0 & \frac{4}{a} & 0 & 0 & - \frac{4}{a b} & - \frac{4}{a c} & 0 & - \frac{4}{a^{2}} & 0 & 0\\0 & 0 & \frac{4}{b} & 0 & - \frac{4}{a b} & 0 & - \frac{4}{b c} & 0 & - \frac{4}{b^{2}} & 0\\0 & 0 & 0 & \frac{4}{c} & 0 & - \frac{4}{a c} & - \frac{4}{b c} & 0 & 0 & - \frac{4}{c^{2}}\\0 & 0 & 0 & 0 & \frac{4}{a b} & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{b c} & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & \frac{4}{a c} & 0 & 0 & 0 & 0\end{matrix}\right]

==> shape-function-info/tet10_reference/B_matrix.tex <==
\left[\begin{matrix}1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\0 & a & 0 & 0 & \frac{a}{2} & 0 & 0 & \frac{a}{2} & 0 & \frac{a}{2}\\0 & 0 & b & 0 & 0 & \frac{b}{2} & 0 & \frac{b}{2} & \frac{b}{2} & 0\\0 & 0 & 0 & c & 0 & 0 & \frac{c}{2} & 0 & \frac{c}{2} & \frac{c}{2}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{a b}{4} & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{a c}{4}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{b c}{4} & 0\\0 & a^{2} & 0 & 0 & \frac{a^{2}}{4} & 0 & 0 & \frac{a^{2}}{4} & 0 & \frac{a^{2}}{4}\\0 & 0 & b^{2} & 0 & 0 & \frac{b^{2}}{4} & 0 & \frac{b^{2}}{4} & \frac{b^{2}}{4} & 0\\0 & 0 & 0 & c^{2} & 0 & 0 & \frac{c^{2}}{4} & 0 & \frac{c^{2}}{4} & \frac{c^{2}}{4}\end{matrix}\right]

==> shape-function-info/tet10_reference/basis_functions.tex <==
\left[\begin{matrix}1\\u\\v\\w\\u v\\u w\\v w\\u^{2}\\v^{2}\\w^{2}\end{matrix}\right]

==> shape-function-info/tet10_reference/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (0, 0, 0) \\
\text{Node 2}: & \quad (a, 0, 0) \\
\text{Node 3}: & \quad (0, b, 0) \\
\text{Node 4}: & \quad (0, 0, c) \\
\text{Node 5}: & \quad (\frac{a}{2}, 0, 0) \\
\text{Node 6}: & \quad (0, \frac{b}{2}, 0) \\
\text{Node 7}: & \quad (0, 0, \frac{c}{2}) \\
\text{Node 8}: & \quad (\frac{a}{2}, \frac{b}{2}, 0) \\
\text{Node 9}: & \quad (0, \frac{b}{2}, \frac{c}{2}) \\
\text{Node 10}: & \quad (\frac{a}{2}, 0, \frac{c}{2}) \\
\end{align*}

==> shape-function-info/tet10_reference/shape_function_derivatives.tex <==
\left[\begin{matrix}- \frac{3}{a} + \frac{4 w}{a c} + \frac{4 v}{a b} + \frac{4 u}{a^{2}} & - \frac{3}{b} + \frac{4 w}{b c} + \frac{4 v}{b^{2}} + \frac{4 u}{a b} & - \frac{3}{c} + \frac{4 w}{c^{2}} + \frac{4 v}{b c} + \frac{4 u}{a c}\\\frac{- a + 4 u}{a^{2}} & 0 & 0\\0 & \frac{- b + 4 v}{b^{2}} & 0\\0 & 0 & \frac{- c + 4 w}{c^{2}}\\\frac{4}{a} - \frac{4 w}{a c} - \frac{4 v}{a b} - \frac{8 u}{a^{2}} & - \frac{4 u}{a b} & - \frac{4 u}{a c}\\- \frac{4 v}{a b} & \frac{4}{b} - \frac{4 w}{b c} - \frac{8 v}{b^{2}} - \frac{4 u}{a b} & - \frac{4 v}{b c}\\- \frac{4 w}{a c} & - \frac{4 w}{b c} & \frac{4}{c} - \frac{8 w}{c^{2}} - \frac{4 v}{b c} - \frac{4 u}{a c}\\\frac{4 v}{a b} & \frac{4 u}{a b} & 0\\0 & \frac{4 w}{b c} & \frac{4 v}{b c}\\\frac{4 w}{a c} & 0 & \frac{4 u}{a c}\end{matrix}\right]

==> shape-function-info/tet10_reference/shape_functions.tex <==
\left[\begin{matrix}1 - \frac{3 w}{c} + \frac{2 w^{2}}{c^{2}} - \frac{3 v}{b} + \frac{4 v w}{b c} + \frac{2 v^{2}}{b^{2}} - \frac{3 u}{a} + \frac{4 u w}{a c} + \frac{4 u v}{a b} + \frac{2 u^{2}}{a^{2}}\\- \frac{u}{a} + \frac{2 u^{2}}{a^{2}}\\- \frac{v}{b} + \frac{2 v^{2}}{b^{2}}\\- \frac{w}{c} + \frac{2 w^{2}}{c^{2}}\\\frac{4 u}{a} - \frac{4 u w}{a c} - \frac{4 u v}{a b} - \frac{4 u^{2}}{a^{2}}\\\frac{4 v}{b} - \frac{4 v w}{b c} - \frac{4 v^{2}}{b^{2}} - \frac{4 u v}{a b}\\\frac{4 w}{c} - \frac{4 w^{2}}{c^{2}} - \frac{4 v w}{b c} - \frac{4 u w}{a c}\\\frac{4 u v}{a b}\\\frac{4 v w}{b c}\\\frac{4 u w}{a c}\end{matrix}\right]

==> shape-function-info/tet10_reference/verification_matrix.tex <==
\left[\begin{matrix}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{matrix}\right]

==> shape-function-info/tet_10/B_inv_matrix.tex <==
\left[\begin{matrix}1 & -3 & -3 & -3 & 4 & 4 & 4 & 2 & 2 & 2\\0 & -1 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0\\0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 2 & 0\\0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 2\\0 & 4 & 0 & 0 & -4 & -4 & 0 & -4 & 0 & 0\\0 & 0 & 4 & 0 & -4 & 0 & -4 & 0 & -4 & 0\\0 & 0 & 0 & 4 & 0 & -4 & -4 & 0 & 0 & -4\\0 & 0 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 4 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 4 & 0 & 0 & 0 & 0\end{matrix}\right]

==> shape-function-info/tet_10/B_matrix.tex <==
\left[\begin{matrix}1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\0 & 1 & 0 & 0 & \frac{1}{2} & 0 & 0 & \frac{1}{2} & 0 & \frac{1}{2}\\0 & 0 & 1 & 0 & 0 & \frac{1}{2} & 0 & \frac{1}{2} & \frac{1}{2} & 0\\0 & 0 & 0 & 1 & 0 & 0 & \frac{1}{2} & 0 & \frac{1}{2} & \frac{1}{2}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{4} & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{4}\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{4} & 0\\0 & 1 & 0 & 0 & \frac{1}{4} & 0 & 0 & \frac{1}{4} & 0 & \frac{1}{4}\\0 & 0 & 1 & 0 & 0 & \frac{1}{4} & 0 & \frac{1}{4} & \frac{1}{4} & 0\\0 & 0 & 0 & 1 & 0 & 0 & \frac{1}{4} & 0 & \frac{1}{4} & \frac{1}{4}\end{matrix}\right]

==> shape-function-info/tet_10/basis_functions.tex <==
\left[\begin{matrix}1\\u\\v\\w\\u v\\u w\\v w\\u^{2}\\v^{2}\\w^{2}\end{matrix}\right]

==> shape-function-info/tet_10/node_locations.tex <==
\begin{align*}
\text{Node 1}: & \quad (0, 0, 0) \\
\text{Node 2}: & \quad (1, 0, 0) \\
\text{Node 3}: & \quad (0, 1, 0) \\
\text{Node 4}: & \quad (0, 0, 1) \\
\text{Node 5}: & \quad (\frac{1}{2}, 0, 0) \\
\text{Node 6}: & \quad (0, \frac{1}{2}, 0) \\
\text{Node 7}: & \quad (0, 0, \frac{1}{2}) \\
\text{Node 8}: & \quad (\frac{1}{2}, \frac{1}{2}, 0) \\
\text{Node 9}: & \quad (0, \frac{1}{2}, \frac{1}{2}) \\
\text{Node 10}: & \quad (\frac{1}{2}, 0, \frac{1}{2}) \\
\end{align*}

==> shape-function-info/tet_10/shape_functions.tex <==
\left[\begin{matrix}2 u^{2} + 4 u v + 4 u w - 3 u + 2 v^{2} + 4 v w - 3 v + 2 w^{2} - 3 w + 1\\2 u^{2} - u\\2 v^{2} - v\\2 w^{2} - w\\- 4 u^{2} - 4 u v - 4 u w + 4 u\\- 4 u v - 4 v^{2} - 4 v w + 4 v\\- 4 u w - 4 v w - 4 w^{2} + 4 w\\4 u v\\4 v w\\4 u w\end{matrix}\right]

==> shape-function-info/tet_10/verification_matrix.tex <==
\left[\begin{matrix}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\end{matrix}\right]
